Physics-Aware Neural Implicit Solvers for multiscale, parametric PDEs with applications in heterogeneous media

We propose Physics-Aware Neural Implicit Solvers (PANIS), a novel, data-driven framework for learning surrogates for parametrized Partial Differential Equations (PDEs). It consists of a probabilistic, learning objective in which weighted residuals are used to probe the PDE and provide a source of {\em virtual} data i.e. the actual PDE never needs to be solved. This is combined with a physics-aware implicit solver that consists of a much coarser, discretized version of the original PDE, which provides the requisite information bottleneck for high-dimensional problems and enables generalization in out-of-distribution settings (e.g. different boundary conditions). We demonstrate its capability in the context of random heterogeneous materials where the input parameters represent the material microstructure. We extend the framework to multiscale problems and show that a surrogate can be learned for the effective (homogenized) solution without ever solving the reference problem. We further demonstrate how the proposed framework can accommodate and generalize several existing learning objectives and architectures while yielding probabilistic surrogates that can quantify predictive uncertainty.

==> section1/1_introduction.tex <==
\section{Introduction}
\label{introduction}


%\psk{parametric PDEs, where do they appear and what are the challenges?}
The core of every simulation before designing or testing an industrial product is solving one or more PDEs. In most state-of-the-art applications, where these PDEs must be inquired multiple times for different setups, such as in optimization under uncertainty problems or in uncertainty quantification applications (forward or inverse), the respective parametric PDEs must be solved. These involve one or more parametric inputs that alternate the behavior of the PDEs and, thus, their solution. Therefore, the goal in such scenarios is ultimately to construct a map between the parametric inputs and the outputs, i.e., the solution of the PDE. In most cases, well-established numerical methods are used to construct the previous map by acquiring the input-output pairs one by one. Even though the quality of these pairs in terms of accuracy is very high, when traditional numerical solvers are used, the same can be said for their computational cost, making the previous approach infeasible, especially for high dimensional parametric PDEs.

Employing inexpensive surrogates capable of approximating sufficiently the solution of parametric PDEs is one approach to addressing the challenge mentioned above. While the cost of the surrogate prediction is often small, it cannot be stated the same for the training cost. For training a surrogate it is necessary to define a learning protocol/objective and a capable model architecture.





%\psk{data-driven strategies, Distinguish between learning protocols/objectives and architectures}
% Many proposed models have attempted to tackle the previous issue, by training physics informed models, which incorporate physical knowledge directly from the PDE itself \cite{karumuri2020simulator}, \cite{zhu2019physics}. However, in very few of these efforts, the training is performed solely by employing physical information from the PDE. This could be partially attributed to the challenges in infusing the plentiful PDE information to the model.


%Usually, such PDEs involve one or multiple parametric inputs In cases where one or more PDEs are required to be inquired multiple times for different setups, such as in optimization under uncertainty problems or in uncertainty quantification applications (forward or inverse)


%In most of the cases, well-established numerical methods are used for obtaining the PDEs solution. Even though these methods give accurate predictions, they are computationally demanding. 

%As a result, in cases where many-query problems are required to be solved, such as in optimization under uncertainty problems or in uncertainty quantification applications (forward or inverse), the computational cost is prohibitive, if conventional numerical methods are used. In such many-query problems the respective parametric PDE needs to be solved. Employing inexpensive surrogates capable of approximating sufficiently the solution of parametric PDEs is one approach for addressing the challenge mentioned above.

==> section1/2_relatedWork.tex <==

\subsection{Related Work regarding the Learning Protocols}
\label{sec:relatedWorkLP}

The learning protocols can be distinguished between data-driven and physics-informed protocols. In data-driven approaches as \cite{lu2019deeponet}, \cite{li2020neural}, \cite{li2020fourier}, the loss function usually involves only one term, which measures the distance between the predicted and the actual solution. Thus, a dataset of inputs-outputs is necessary for training in the previous cases. Although data-driven methods have a slightly faster and more stable training phase, obtaining the dataset can be computationally demanding or even infeasible for some difficult, high-dimensional parametric PDEs since the forward model (expensive numerical solver) must be called many times. Moreover, training a model strictly with labeled data will result in one with mostly interpolative and rarely extrapolative behavior. The second characteristic would be more desirable since the model should retain its predictive capabilities even for parametric inputs outside the training space.

On the other side of the spectrum lie physics-informed learning protocols for training surrogates \cite{raissi2017physics}, \cite{wang2021learning}. Even though the training phase requires no labeled data and the information is acquired during training, infusing the plentiful PDE information into the model is much more involved. Hence, in very few of these efforts, the training is performed solely by employing physical information from the PDE. The loss function frequently consists of multiple terms, the most important of which is the one that measures the distance of the PDE residuals \cite{nabian2018deep}, \cite{karumuri2020simulator} or energy functionals \cite{zhu2019physics}, \cite{rixner2021probabilistic}, \cite{goswami2020transfer} from zero. As a result, the objective function changes with the parametric PDE problem for which the surrogate is to be trained. In general, training physics-informed surrogates is faster since there is no need for labeled data and their predictions tend to have higher accuracy on previously unseen inputs.

\subsection{Related Work regarding the Architecture}
\label{sec:relatedWorkAR}

In cases where the dimension of the problem is low to medium, well-tested - traditional architectures exist for constructing inexpensive prediction tools. Some of the well known ones include Radial Basis Functions \cite{regis2013}, Gaussian Process Regression \cite{BILIONIS20125718}, \cite{CHEN2015291}, \cite{Martin2005}, and polynomial chaos expansion \cite{Xiu2002}, \cite{Najm2009}, \cite{ernst2012}. Despite some recent efforts to scale up the capabilities of Gaussian Processes in higher dimensional problems \cite{atkinson2019}, \cite{van2017}, the above-mentioned methods still struggle in such cases. The problem with higher dimensional problems lies in the fact that the number of data points required to accurately approximate the solution grows exponentially with the dimension of the problem, which is also known as the Curse of Dimensionality \cite{grohs2018}.

One obvious approach for combating this issue is to employ dimensionality reduction methods, which can be considered as an alternative architecture. Traditional architectures based on the  Karhunen-Lo\'eve Expansion (KLE) \cite{ghanem1999stochastic}, Principal Component Analysis (PCA) \cite{abdi2010principal} and it's evolved form KPCA \cite{ma2011kernel}, were some of the first ones to be embedded in the discussed models. The above tools are utilized in Reduced-Basis (RB) models \cite{quarteroni2015reduced}, \cite{hesthaven2016certified}, \cite{grepl2007efficient}, where paired data can be acquired inexpensively from solving a lower dimensional problem, which originates from projecting onto the principal directions of high fidelity one. An alternative method that was introduced for taking the model output information into account was the Active Subspace (AS) method \cite{constantine2014active}, \cite{constantine2014computing}, which relies on an empirical approach for performing the eigendecomposition. Leveraging the power of deep learning was maybe the most recent effort towards this direction, in which various learning strategies were tested \cite{kani2017dr}, \cite{guo2018reduced}.

Furthermore, the recent advances in deep learning \cite{Goodfellow-et-al-2016}, triggered a big effort towards the utilization of Deep Neural Networks for solving efficiently problems consisting of parameteric PDEs \cite{han2018solving}, \cite{sirignano2018dgm}, \cite{li2017deep}. Combining the potential of DNNs with dimensionality reduction techniques, as the ones above, was demonstrated in high dimensional heterogeneous media problems in \cite{grigo2019bayesian}, \cite{yang2019conditional}, \cite{zhu2018bayesian}, \cite{mo2019deep}. In the work of \cite{raissi2017physics}, \cite{yang2019adversarial}, \cite{kaltenbach2020incorporating}, \cite{rixner2021probabilistic}, \cite{raissi2018hidden}, \cite{yu2018deep} the loss function used for training the model was consisted of both labeled data and physical information from the governing equations in the form of residuals. A detailed taxonomy \cite{kim2021knowledge} and review regarding the application of deep-physics-informed models for solving various problem as well as PDEs is documented in \cite{frank2020machine}, \cite{karniadakis2021physics}. 

One of the latest and most promising advancements in learning the outputs of parametric PDEs regarding the used architecture is the Deep-Operator based framework \cite{kovachki2021neural}. Such frameworks are used to learn functional mappings between the input-solution spaces of the PDEs. The first data-driven neural operator developed was the DeepONet \cite{lu2019deeponet} (physics informed \cite{wang2021learning}) followed by the improved Graph Neural Operator (GNO) \cite{li2020neural}. To solve the instability issues of GNOs the Fourier Neural Operator (FNO) was introduced, where the architecture involves multiple Fourier Transforms and their inverses \cite{li2020fourier}, \cite{li2021physics}. The latest neural operator variant utilizes the Wavelet transformation (WNO) \cite{tripura2022wavelet}, which was employed to tackle the shortcomings of the FNO regarding the lack of information about the spatial resolution \cite{bachman2000fourier}. An effort to provide probabilistic predictions for the outputs after learning the map was done in \cite{garg2022variational} in a data-driven approach.


==> section1/3_proposedFramework.tex <==
\subsection{The Proposed Framework}
\label{sec:proposedFramework}
Learning parametric PDEs is a small data problem \cite{rixner2021probabilistic} and thus the majority of the information required for training should originate from the physical information of the PDE. Furthermore, we think that a probabilistic approach is a superior tool in such problems, since the uncertainty of the final prediction can be quantified, while the quality of the information is better sustained, when dimensionality reduction methods are utilized in the framework.

%Another important quality that we value in a framework is the capability of handling problems defined in irregular domains where traditional numerical tools suffer from instabilities or large computational times.

In \cite{zhu2019physics}, we introduced a target probability density that incorporated the governing equations. In this work, we revisit such formulations from the point of view afforded by the concept of {\em virtual observables} (\cite{kaltenbach2020incorporating,rixner2021probabilistic}). This allows us to augment the family of distributions considered but, more importantly, to propose a new algorithm that is more efficient in ingesting information from the governing PDE. This algorithm employs weighted residuals in order to incorporate the governing PDE in the learning objectives. Each of the weighting functions employed in a weighted residual corresponds to a different probe that furnishes different type or amount of information regarding its solution and its dependence on the parametric input. 

In the context of multiscale PDEs where the solution contains high frequency/wavenumber fluctuations that must be accounted for even if one is only interested in capturing the dominant low frequency/wavenumber ones, various enhanced NN-based architectures have been proposed \cite{liu_mitigating_2023,rixner2021probabilistic}. 
While these might be effective for some problems, the number of parameters grows exponentially with the dimension of the problem. It is our belief that such methods postpone addressing the fundamental problem of identifying low-dimensional bottlenecks that enable accurate predictions even in high-dimensional or multiscale settings. As we have demonstrated in  previous work \cite{grigo_physics-aware_2019,rixner2021probabilistic} retaining some of the physical structure can be extremely advantageous in this direction. We do not dismiss the NN-based architectures that have been proposed and in fact, as we discuss in the sequel, the majority of them can be readily integrated in the probabilistic framework advocated in this paper.

%In this paper, we propose a probabilistic framework to combat the aforementioned challenges that emerge when solving high dimensional parametric PDEs. During the training of the model, the information originates exclusively from the weak form of the respective PDE. The physical information is extracted efficiently from the weak formulation by using the weight functions as probes. At each iteration of the proposed algorithm, the information is introduced by maximizing the residual of the weak form, while a Stochastic Variational Inference \cite{hoffman2013stochastic, paisley2012variational} scheme is employed in order to train the approximate variational distribution. The previous combination led to three different novel algorithms based on stochastic gradient ascent/descent schemes. 

%The aforementioned methods are enhanced by various deep learning-based, dimensionality reduction routines, which are trained simultaneously with the main algorithm. First and foremost, these are used for extracting the lower dimensional inputs that are most expressive of the high-dimensional outputs, for the probabilistic surrogate's first and higher uncertainty moments. Secondly, these features contribute to the acceleration of the algorithm by reducing the number of trainable parameters. 

\bigbreak





==> section1/4_contributions.tex <==
\subsection{Our Contributions}
The novel characteristics of the proposed approach consist of the following:

\begin{itemize}

\item A physics-inspired architecture is introduced that involves an implicit coarse-grained solver, which serves as an efficient informational bottleneck. This, in turn, improves the generalization-extrapolation capabilities, while significantly reducing the complexity and the total number of parameters of the model, leading to faster and more stable training.

\item The framework efficiently ingests the PDE using weighted residuals in which case the associated weight functions serve as probes. Furthermore, it provides probabilistic predictions, which are essential, because the coarse-grained solver cannot fully resolve the solution. In our knowledge, the above-described method is one of the few, if not the first, to provide uncertainty bounds on the solution when learning parametric PDE maps by only using information from the PDE (physics-informed learning).

%\item The methods provide more accurate mean predictions from state-of-the-art physics-informed methods (\textcolor{red}{XX \% more accurate than PINO in high dimensional problems.})
\item Because of the above components, the proposed framework can provide accurate out-of-distribution predictions for a wide variety of boundary conditions and effective properties of the underline input, something that isn't true for other state-of-the-art models (PINO \cite{li2021physics}).
%\item The number of residual calculations required for the same level of accuracy in the predictions is significantly reduced compared to other state-of-the-art models (PINO).
\item Last but not least, we propose a new method for successfully capturing the dominant low-frequency fluctuations of the solution manifold in a challenging multi-scale setup, by using the residual as the only source of information for training. To our knowledge, this is the first model to ever achieve the above. The performance-to-cost ratio in such cases is far higher than the one achieved by state-of-the-art neural operators.

\item Generalization of several existing physics-informed schemes which can be accommodated as special cases in the general framework proposed.
\end{itemize}

%\psk{The review of the state-of-the-art should be structured along the two threads i.e. learning objectives and architectures. The primary focus should be on the former as your contributions lie (primarily) there. I'd classify the "dimensionality reduction" techniques under architectures unless they affect the learning objectives which would definitely NOT be the case if they are done offline i.e. separated from learning the surrogate. As for the different architectures you can claim that they can be used (some or all) in your framework as well. Please also make reference to our prior work especially the one that pertains to virtual observables. }


% \psk{
% \noindent \textbf{Remarks:} (to incorporate later)
% \bi
% \item In \cite{zhu2019physics} we introduced a target probability density that incorporated the governing equations. In this work, we revisit such formulations from the point of view afforded by the concept of {\em virtual observables} (\cite{kaltenbach2020incorporating,rixner2021probabilistic}). This allows us to augment the family of distributions considered but more importantly to propose three algorithms which are more efficient in ingesting information from the governing PDE.
% \item In this work we use weighted residuals in order to incorporate the governing PDE in the learning objectives. Each of the weighting functions employed in a weighted residual corresponds to a different probe that furnishes different type or amount of information regarding its solution and its dependence on the parametric input. 

% \item In context of multiscale PDEs where the solution contains high frequency/wavenumber fluctuations that must be accounted for even if one is only interested in capture the dominant low frequency/wavenumber ones, various enhanced NN-based architectures have been proposed \cite{liu_mitigating_2023,rixner2021probabilistic}. While these might be effective for some problems, the number of parameters grows exponentially with the dimension of the problem. It is our belief that such methods postpone addressing the fundamental problem of identifying low-dimensional bottlenecks that enable accurate predictions even in high-dimensional or multiscale settings. As we have demonstrated in  previous work \cite{grigo_physics-aware_2019,rixner2021probabilistic} retaining some of the physical structure can be extremely advantageous in this direction. We do not dismiss the NN-based architectures that have been proposed and in fact, as we discuss in the sequel, the majority of them can be readily integrated in the probabilistic framework advocated in this paper.

% \ei
% }

==> section2/10_predictiveMetrics.tex <==
\subsection{Predictions}

After training has finished, the density $q_{\bpsi}(\by|\bx)$ that has been obtained can be used for providing predictions. Samples can be drawn from $q_{\bpsi}(\by|\bx)$ because of its Gaussian form. For any given input $\bx$, the mean coefficients of the solution are given from Equation \eqref{eq:formOfmeanPrediction}. The previous samples and the mean coefficients can be easily converted to the respective fields by using the representation shown in Equation \eqref{eq:trialSolRepresentation} (see subsection \ref{sub:2D_Darcy}). The variance of the predicted field can be determined empirically from the previous samples, and in turn, one can obtain the upper and lower uncertainty bound of the solution for any given $\bx$. The process for obtaining probabilistic predictions is shown in Algorithm \ref{alg:MakingPredictions}.

\begin{algorithm}[H]
% \caption{Simple Description of the Learning Algorithm.}

%Given a single input $\bx$ for which we wish to make a prediction:\;

\begin{algorithmic}[1]
    \State {$u_{\mu}(\bs{s}) \leftarrow \sum_{i=1}^{N_{\eta}} \mu_{\bpsi} (\bx)_i \eta_i(\bs{s})$} \Comment{Mean Solution Field}
    \For{$j=1$ to $J$}
    \State {Sample $\by^{(j)} \sim q_{\bpsi}(\by|\bx)$\;}      \Comment{$q_{\bpsi}(\by|\bx)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \boldsymbol{\Sigma}_{\bpsi})$}
    \State {$u^{(j)}(\bs{s}) = \sum_{i=1}^{N_{\eta}} y_i^{(j)} \eta_i(\bs{s})$} \Comment{Reconstruction of the Solution fields (see Equation \ref{eq:trialSolRepresentation})}
    \EndFor
    \State $u_{\sigma}(\bs{s}) \leftarrow \sqrt{ \sum_{j=1}^J \frac{\left( u^{(j)}(\bs{s}) - u_{\mu}(\bs{s})\right)^2}{J-1}}$ \Comment{Standard Deviation of the Solution Field}
    \State $u_{U}(\bs{s}) \leftarrow u_{\mu}(\bs{s}) + 2 u_{\sigma}(\bs{s})$ \Comment{Upper Uncertainty Bound Field}
    \State $u_{L}(\bs{s}) \leftarrow u_{\mu}(\bs{s}) - 2 u_{\sigma}(\bs{s})$ \Comment{Lower Uncertainty Bound Field}
    
\end{algorithmic}
\caption{Making Predictions for a single input $\bx$}
%\caption{Assuming $q_{\bpsi}(\bx,\by)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T)~\mathcal{N}\left(\bx | \bs{0}, \bs{I}\right)$ }
\label{alg:MakingPredictions}
%\psk{Algorithms should come after the full model has been presented}
\end{algorithm}

To assess the performance of the proposed model and compare it objectively with other state-of-the-art models, we consider a validation dataset $\mathcal{D}_v = \{ \mathbf{x}^j, \mathbf{y}^j \}_{j=1}^{N_j}$ consisting of $N_j$ input-output pairs, which were obtained by using a conventional FEM solver on a fine mesh. Subsequently, the following metrics will be employed:

\textbf{Coefficient of Determination $R^2$:}
The coefficient of determination is a widely used metric \cite{coeffDetermZhang} to quantify the accuracy of point estimates and it is defined as follows

\begin{equation}
R^2 = 1 - \frac{\sum_{j=1}^{N_j} \| \by_j - \mu(\bx_j) \|_2^2}{\sum_{j=1}^{N_j} \| \by_j - \bar{\by} \|_2^2}
\end{equation}

where $\mu(\bx_j) = \mathbb{E}_{q_{\bpsi}(\by | \bx)} \left[ \by \right]$ is the mean of the predictive posterior $q_{\bpsi}(\by|\bx)$ of our trained model for each point $\bx_j$ and $\bar{\by} = \frac{1}{N_j} \sum_{j=1}^{N_j} \by_j$ is the sample mean of the validation dataset. According to the previous metric, the best possible prediction accuracy is attained when $R^2=1$. It is noted that negative $R^2$ values are also valid since the second term is merely weighted (not bounded) by the empirical variance of the validation dataset.

\textbf{Relative $L_2$ Error $\epsilon$:} The relative $L_2$ error is commonly used as an evaluation metric for comparisons between state-of-the-art surrogate models for stochastic PDEs \cite{zhu2019physics, lu2022comprehensive, wang2021learning}. The definition is given by

\begin{equation}
\epsilon = \frac{1}{N_j} \sum_{j=1}^{N_j}\frac{ \| \by_j - \mu(\bx_j) \|_2}{\| \by_j \|_2}.
\end{equation}
%\textbf{Enveloping Score $M_e$:}


%\psk{Don't u show predictive estimates based on $q(\by|\bx)$ as well? An algorithm should be added that explains how these predictive estimates are generated see e.g. \cite{rixner2021probabilistic} Alg. 2.}




==> section2/1_methodology.tex <==
\section{Methodology}

%\psk{if $\by$ is a vector, $\mathcal{L}$ cannot be a differential operator. You need to distinguish between the continuous version (strong form) and the discretized. The latter can come after you introduce the weighted residuals. You have do be careful in defining densities on function spaces, see e.g. \cite{alberts_physics-informed_2023,
%chen_solving_2021}} \mc{Thank you for the comment. I tried to create a more solid definition. Do you think that this is now solid or do I need to correct it further?}

We are concerned with parametrized PDEs which can be generally written as:
%The general problem for which the framework will be developed, is described in the following equations:


\be
\begin{array}{ll}
\mathcal{L}(c(\bs{s,x}), u(\bs{s}))=0,~~~ \bs{s} \in \Omega & \textrm{((non)linear differential operator)} \\
\mathcal{B}(c(\bs{s,x}), u(\bs{s}))=0, \quad \bs{s} \in \pa \Omega & \textrm{(boundary-conditions  operator)} \\
\end{array}
\ee
%
where $\bs{s}$ denotes space, $\Omega \subset \RR^{d_s}$ the problem domain,  $c(\bs{s,x})$ denotes an input function parametrized  by $\bx \in \mathcal{X} \subset \RR^{d_x}$ (e.g. material property field) and  $u(\bs{s})$ the sought solution to the boundary value problem above. 
In the following we adopt a discretized representation of the solution i.e. $u(\bs{s})\xrightarrow[]{\text{discretize}} \by$ where $\by \in \mathcal{Y} \subset \RR^{d_y}$. We assume that that the adopted discretization is fine enough to provide an acceptable approximation to the actual solution which in general implies that $dim(\by)>>1$. The vector $\by$ could represent coefficients with respect to a given set of functions (e.g. FE shape functions, Radial Basis Functions,  Fourier, Wavelet) or the weight/biases of a  neural network.  We adopt a finite-dimensional, albeit potentially high-dimensional, representation of the input and output although this can be relaxed +++++++\cite{fanaskov_spectral_2023}.



% \in \mathcal{Y}$ is the unknown/solution function of the parametric PDE. We denote with $c(\bs{s}, \bx)$ and $u(\bs{s}, \by)$ some discretized versions of $c(\bs{s})$ and $u(\bs{s})$ respectively, where $\bx$ is the input vector $\bx \in R^{d_{\bx}}$ and $\by$ the output/unknown vector $\by \in R^{d_{\by}}$. 

We aim at  developing a {\em probabilistic} surrogate which will be expressed in the form of a density $q(\by |\bx)$ that can predict the (discretized) solution for any input $\bx$ and especially in the high-dimensional setting i.e. when $d_x,d_y>>1$.
We note that the predictive uncertainty in this case is not due to aleatoric stochasticity in the governing equations (although such cases can be accommodated as well) but of epistemic nature due to the use of partial, and hopefully small, data in constructing this surrogate as explained in the sequel. 
%
%In most cases of practical interest, the dimensions of the inputs and outputs are high, i.e. $d_{\bx}, ~d_{\by} >> 1$, and the times that the above equations need to be inquired are high as well (e.g. optimization under uncertainty or forward/inverse uncertainty quantification problems). The goal of the proposed framework is to train an approximate predictive surrogate $q(\by| \bx)( \bs{s})$, which will be capable of providing computationally inexpensive probabilistic predictions about $\by$ for any given $\bx$ at the requested spatial coordinates $\bs{s}$. In other words, we attempt to learn an approximation of the map $\mathcal{X} \rightarrow \mathcal{Y}$ between the functions $c(\bs{s})$ and $u(\bs{s})$.


==> section2/2_strongWeakForm.tex <==

\subsection{Strong and Weak of a boundary-value problem}
\label{sec:SWform}

We view the governing PDE as an infinite source of information which we probe with the help of {\em weighted residuals}. These constitute the (virtual) data with which we attempt to train our surrogate.
In order to illustrate this concretely and clearly, we use as an example a linear, elliptic PDE. The methodological elements can then be generalized to other types of PDEs.
In particular, we consider the boundary value problem:
%For the derivation of the framework, the strong form of the parametric PDE should be firstly written. As an example, we will use a simple parametric Elliptic PDE with its respective boundary conditions 

\be
\begin{array}{rl}
 \nabla (-c(\bs{s}, \bx) \nabla u(\bs{s}))=g, & \bs{s} \in \Omega\\
 u(\bs{s})=u_0, &   \bs{s} \in \Gamma_u \\
 -c(\bs{s}, \bx) \nabla u(\bs{s}) \bs{n}=q_0, &  \bs{s} \in \Gamma_q =\pa \Omega - \Gamma_u
\end{array}
\label{eq:DarcyFlowEquation}
\ee
%\psk{$\by$ are not parameters that $u$ depends on but the representation of $u$ upon discretization}
where $c(\bs{s}, \bx)$ is a (random) conductivity/permeability/diffusivity  field which depends on the parameters $\bx$. %, % $g$ is the term of the external forces applied, $u(\bs{s})$ is the solution field, $\Omega$ is the definition space, 
We denote with $\Gamma_u$ and $\Gamma_q$ the parts of the boundary  where Dirichlet and Neumann conditions are respectively defined. The symbol $\bs{n}$ indicates the outward vector, which is normal to the boundary, while the $u_0$ and $q_0$ denote the prescribed values. % of at the boundaries, where Dirichlet and Neumann conditions are respectively applied.

We employ candidate solutions $u_{\by}$ which are represented by the finite-dimensional  $\by \in \RR^{d_y}$ as discussed above and which are assumed to a priori satisfy the Dirichlet BCs \footnote{This requirement is consistent with traditional derivations but can be readily relaxed or removed in our formulation.}. These are combined with weighting functions $w(\bs{s}) \in \mathcal{W}$ which are assumed to be zero at the Dirichlet boundary i.e. $w(\bs{s})|_{\bs{s} \in \Gamma_u}=0$.
%For the solution field $u(\bs{s})$ we select the following representation:
%
%\be
%u(\bs{s})=\sum_{j=1}^n y_j \phi_j(\bs{s}),
%\label{eq:trialSolRepresentation}
%\ee

%\noindent where $\bs{y}$ are the output vector (coefficients of the solution representation), $n=dim(\by)$ and $\phi_j(\bs{s})$, are the corresponding shape/basis functions. If $w$ denotes appropriate weight functions such that $w(\bs{s})|_{\bs{s} \in \Gamma_u}=0$, then the weak form of the above equation will be \cite{finlayson_method_1972}
By employing integration-by-parts \cite{finlayson_method_1972} and for each such $w(\bs{s})$ we obtain the weighted residual:
\be
r_w(\by,\bx) = 0= \int_{\Gamma_q} w~ q_0 ~d\Gamma+\int_{\Omega} \nabla w~ c(\bs{s}, \bx) ~\nabla u_{\by}~ d\bs{s} -\int_{\Omega} w~ g ~d\bs{s}.
\label{eq:weak1}
\ee

\noindent We note that depending on the choice of the weight functions $w$ (at least) six methods (i.e. collocation, sub-domain, least-squares, (Petrov)-Galerkin, moments) arise as  special cases \citep{finlayson_method_1972}. As it will become apparent in the sequel, the weighted residuals are used as data sources and not in  the traditional sense, i.e. to derive a discretized system of equations  for the approximate solution of the problem. Hence we would be at liberty to consider alternate or even non-symmetric versions with respect to $u$ and $w$ as for example by applying  further integration-by-parts which would  lead to expressions with  lower-order derivatives of the candidate solution $u_{\by}$.

%\psk{
%\noindent \textbf{Remarks:}
%\begin{itemize}
%\item Depending on the choice of the weight functions $w$ (at least) six methods (i.e. collocation, sub-%domain, least-squares, (Petrov)-Galerkin, moments) arise as  special cases \citep{finlayson_method_1972}.
%\item Since weighted residuals are not employed here in the traditional sense and in order to obtain %approximate solutions to the PDE, we are at liberty to consider alternative versions. For example, it is %not necessary that the final form is symmetric with respect to $u$ and $w$ but integration-by-parts could %further be employed in order to obtain expressions that contain lower-order derivatives of the candidate %solution $u$. 
%\end{itemize} }

==> section2/3_virtualObservables.tex <==

\subsection{ Virtual Observables and Virtual Likelihhod} \label{infusingVirtualObservables}

Rather than solving the governing equations multiple times for different values of $\bx$ in order to obtain a {\em labeled} training dataset (i.e. pairs of $(\bx,\by)$) %In the case of training with labeled data, the above PDE should be inquired many times for different inputs $\bx$ and spatial coordinates $\mathbf{s}$ in order to create the necessary pairs of data for the training. In our formulation, this process is completely avoided 
we treat weighted residuals as in \refeq{eq:weak1} as {\em virtual observables} \cite{kaltenbach2020incorporating}.
In particular, given   $N$ distinct weighting function $w_j$ and the corresponding residuals $r_{w_j}(\by,\bx)$, we consider that their values $\hat{r}_j$ have been {\em virtually} observed and are equal to $0$ i.e. the solution pairs $(\bx,\by)$ perfectly satisfy them. The {\em virtual} observables $\hat{\bs{R}}=\{ \hat{r}_j=0 \}_{j=1}^N$ imply a {\em virtual} likelihood which is assumed to be of the form: 
%are assumed to be equal to $0$ and relate to the  $r_{w_j}$ as follows:
%This is achieved by considering $N$ different weight functions $w_j$ and their corresponding residuals $r_{w_j}$. Thus, the training dataset will be given by the associated virtual observables $\hat{\bs{R}_N}=\{ \hat{r}_j=0 \}_{j=1}^N$. In other words, the residuals of the respective weight functions from equations (\ref{weak1}) are assumed to be equal to zero. The virtual data needs to be introduced to the probabilistic framework via the likelihood. Hence, the virtual observables are distorted with noise, as shown in the following equation

%\be
%0=\hat{r}_j=r_{w_j}(\by, \bx)+\frac{1}{\sqrt{\lambda}} \epsilon_r, \qquad \epsilon_r \sim p(\epsilon_r),
%\ee
%
%where $\lambda$ is the precision of the noise. Even though a Gaussian noise $\left( p(\epsilon_r)=\frac{1}{\sqrt{2 \pi}}exp{\left(-\frac{\epsilon_r^2}{2}\right)}\right) $ is most commonly used for constructing the likelihood, after experiments, it was concluded that a Laplacian noise $\left( p(\epsilon_r)=\frac{1}{2}exp\left(-|\epsilon_r|\right) \right)$ leads to faster training. This might be happening, because the partial derivatives $\frac{\partial r_{w_j}}{\partial \bx}$ or $\frac{\partial r_{w_j}}{\partial \by}$ are better behaved in the latter case. In turn this implies a {\em virtual} likelihood $p(\hat{\bs{R}} | \by, \bx)$\footnote{dependence on $\lambda$ is omitted} such that:
\be
\begin{array}{ll}
 p(\hat{\bs{R}} | \by, \bx) & =\prod_{j=1}^N p(\hat{r}_j=0 | \by, \bx) \\
 & = \prod_{j=1}^N \frac{\lambda}{2}  e^{ - \lambda |r_{w_j}(\by,\bx)|}
 %Laplace(\hat{r}_j=0 | r_{w_j}(\by, \bx), \lambda^{-1}) 
 \end{array}
\label{eq:virtuallike}
\ee
%
The role of the hyper-parameter $\lambda$ is significant as it controls how the likelihood of a pair $(\bx,\by)$ will decay if the corresponding residuals $r_{w_j}((\by, \bx)$ are different from zero. We note that alternative forms of the virtual likelihood are also possible (e.g. Gaussian)  but the form above was found to yield better results in the numerical experiments performed.  The role of the virtual observables/likelihood is to  provide information from the governing equations {\em without} having to solve them. We discuss in the sequel how this virtual likelihood can be used to learn a surrogate of the PDE solver and how this can be carried out by evaluating a few residuals at a time (i.e. without ever solving the weak form). 
%were carried out 
%On the other side, $r_{w_j}(\by, \bx)$ is the location parameter of the Laplacian distribution, obtained inexpensively by integrating numerically the equations (\ref{weak1}).


==> section2/4_elboDerivation.tex <==

\subsection{Learning surrogates as probabilistic inference}
\label{sub:probInference}

Let $p(\bx)$ be a density on the parametric input. In the case of a random input this is directly furnished by the problem definition. For deterministic problems this could simply be a uniform density over the domain of possible values of $\bx$. 
We complement this with a {\em prior} density $p(\by|\bx)$. In the ensuing numerical experiments a vague, uninformative  such  prior was selected. We note that its role is not provide a good approximation of the sought output $\by$ given an input $\bx$ as this is to be achieved by  the {\em posterior} discussed later. Naturally though,  informative priors could accelerate inference. Parametrized versions could also be employed as e.g. in \cite{rixner2021probabilistic}  and the parameters can be fine-tuned as discussed in the the Remarks at the end of section \ref{sub:probInference} +++++.

The combination of the aforementioned prior densities with the virtual likelihood of \refeq{eq:virtuallike} in the context of  Bayes' rule leads to the {\em joint} posterior $p(\bx, \by | \hat{\bs{R}})$ as follows:
%After obtaining the likelihood, the posterior can be written by using Bayes Rule

\be
\begin{array}{ll}
p(\bx, \by | \hat{\bs{R}}) & =\cfrac{ p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx) }{ p(\hat{\bs{R}}) } \\
%& \propto p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx)  
\end{array}
\label{eq:postint}
\ee
We  emphasize the posterior above is defined on the {\em joint} space of inputs and outputs. Apart from the effect of the prior, it assigns highest probability to pairs of $\bx$ and $\by$ that achieve  $0$ residuals as is the case when they are a solution pair of the boundary value problem.

%where the term $p(\hat{\bs{R}})$ is the evidence and the term $p(\by |\bx) p(\bx)$ is a properly selected prior. The last could be just an uninformative prior in the simplest case, but if mildly parameterized, such a prior could significantly accelerate the convergence of the algorithm. For example, this prior could be a coarse-grained component of the scheme that quickly restricts the algorithm from exploring non-physical solutions.

Since the posterior is generally intractable, we advocate a Variational Inference scheme (refs) \mc{\cite{hoffman2013stochastic,paisley2012variational}?}
 i.e. we seek an approximation from a parametrized family of densities $q_{\bpsi}(\bx,\by)$ by minimizing the Kullback-Leibler divergence with the exact posterior above. 
 If $\bpsi$ denotes the tunable parameters, this is equivalent (refs) \mc{\cite{blei2017variational}?} to maximizing the Evidence Lower BOund (ELBO) $\mathcal{F}(\bpsi)$ to the log-evidence $\log p(\hat{\bs{R}})$ i.e.:
%The posterior could be approximated by using SVI \cite{paisley2012variational}, \cite{hoffman2013stochastic}. Starting from the Evidence, on can derive the ELBO as shown in the following equation:

\be
\begin{array}{ll}
 \log p( \hat{\bs{R}}) & = \log \int   p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx) ~d\by ~d\bx \\
 & \ge \left< \log \cfrac{   p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx) }{q_{\bpsi}(\bx,\by)} \right>_{q_{\bpsi}(\bx,\by)} \\
 & =\mathcal{F} (\bpsi) %= ELBO_{\bpsi}
 \end{array}
 \label{eq:logevi}
\ee
where the brackets $<.>_{q}$ indicate an expectation with respect to $q$. 
Substitution of \refeq{eq:virtuallike} 
 in the expression above leads to:
 %where variational approximation $q$ is trained by using the parameters $\bpsi$. Furthermore, equation \ref{eq:logevi} could be further expanded in the two following terms

\be
\begin{array}{ll}
 \mathcal{F} (\bpsi) &  = N\log \frac{\lambda}{2} - \lambda \sum_{j=1}^N \left< |r_{w_j}(\by,\bx)|\right> _{q_{\bpsi}(\bx,\by)}+ \left< \log \cfrac{p(\by |\bx) p(\bx) }{q_{\bpsi}(\bx,\by)}\right>_{q_{\bpsi}(\bx,\by)} \\
& = N\log \frac{\lambda}{2} - \lambda \sum_{j=1}^N \left< |r_{w_j}(\by,\bx)|\right> _{q_{\bpsi}(\bx,\by)}-KL\left(q_{\bpsi}(\bx,\by) ||  p(\by |\bx) p(\bx) \right) \\
 \end{array}
\label{eq:elbon}
\ee
Apart from the first term, which is irrelevant when $\bs{\lambda}$ is fixed, we note that the objective above promotes $q_{\bpsi}$ that simultaneously  minimize (on average) the absolute values of the $N$ residuals considered while minimizing the KL-divergence from the prior density adopted. 

\noindent \textbf{Remarks:}\\
\bi
\item The KL-divergence term in \refeq{eq:elbon} can be thought of  as a regularization or penalty term, which  nevertheless arises naturally in the Bayesian framework adopted.  In other physics-informed schemes that have been proposed (refs), ad-hoc parameters are generally selected as relative weights of these two terms. Similarly, alternative forms of virtual likelihoods  can give rise to the exact expressions found in competitive schemes. E.g. the use of a Gaussian likelihood would yield the sum of the {\em squares} of the $N$ residuals in the ELBO.
%
\item Furthermore such schemes generally employ collocation-type residuals in the physics-informed term \cite{raissi2019physics,lu2019deeponet,wang2021learning,li2021physics,nabian2018deep,zang2020weak}, which in our formulation arise as a special case  when the weight functions considered take the form of Dirac-deltas i.e. $w_j(\bs{s})=\delta(\bs{s}-\bs{s_j})$ where $\bs{s}_j$ correspond to the collocation points.
%
\item More importantly, by finding the optimal $q_{\bpsi}$ we obtain a {\em probabilistic surrogate} that is capable of providing probabilistic predictions of the solution $\by$ for any input $\bx$. Since the form of $q_{\bpsi}$ is critical to the accuracy of the proposed scheme we defer detailed discussions to Section \ref{sec:ApproximatingDensity}. As a final note we mention that if a degenerate $q_{\bpsi}$ is selected in the form of a Dirac-delta, then one obtains a {\em deterministic} surrogate as is the majority of the ones proposed in the literature \cite{raissi2019physics,lu2019deeponet,yu2018deep}. 
\ei
 



%To find the best possible approximate posterior $q_{\bpsi}(\bx,\by)$, both terms need to be minimized. The second one implies that the KL divergence of the approximate posterior from the prior needs to be minimized. The first term, on the other hand, states that the mean absolute value of the residuals should be minimized. In most physics-informed methods \cite{wang2021learning}, \cite{li2021physics}, the collocation method is used, which is a special case of the weighted residual method above. The form of the weight functions used in these cases is 

%\be
%w_j = \delta(\mathbf{s} - \mathbf{s}_j)
%\ee

%which has the property

%\be
%\int_{\Omega} r_j \delta(\mathbf{s} - \mathbf{s}_j) d\mathbf{s} = \left. r_j \right|_{\mathbf{s}_j}
%\ee


%After a second inspection of the first term, a question that naturally arises, is which and how many weight functions should be used to inquire the PDE as efficiently as possible. The following subsection describes a simple but efficient algorithm for doing so.


==> section2/5_randomResidualAlgorithm.tex <==
\subsection{Randomized Residual Algorithm}
\psk{Probably this should be discussed with the other algorithmic aspects as it is another MC approximation}
The evaluation and, more importantly,  the maximization of the ELBO $\mathcal{F}(\bpsi)$ requires the computation of the expectations with respect to $q_{\bpsi}$ of the absolute values of the $N$ weighted-residuals appearing in the virtual likelihood. We note that the evaluation of a weighted residual involves the computation of an integral over the problem domain (see e.g. \refeq{eq:weak1}) but not the solution of the PDE. These integrations can be carried out using deterministic or Monte-Carlo-based numerical integration schemes (refs). Furthermore if the weight functions have support on a subset of the problem domain $\Omega$ additional efficiencies can be achieved in the numerical integration. 


Independently of the particulars, it is readily understood that  as $N$ increases so does the information we extract from the governing PDE but so does also the computational effort. 
In order to improve the computational efficiency of these updates we propose a Monte Carlo approximation of the pertinent term in the ELBO in \refeq{eq:elbon}. In particular
%The sum, which appears in equation (\ref{eq:elbon}) can be approximated by Monte Carlo as follows

\begin{equation}
\sum_{j=1}^N \left< |r_{w_j}(\by,\bx)| \right> _{q_{\bpsi}(\bx,\by)} \approx \frac{N}{M} \sum_{k=1}^M \left< |r_{w_{j_k}}(\by,\bx)| \right> _{q_{\bpsi}(\bx,\by)}, ~\text{where } j_k \sim Cat\left(N,\frac{1}{N}\right)
\end{equation}
In essence, we sample at random and with equal probability $M<N$  weight functions out of the $N$ and use them to approximate the sum. As $M$ increases so does the Monte Carlo error decrease but so does the computational effort decrease. Since the Monte Carlo estimator is unbiased, even $M=1$ i.e. evaluating a single residual is sufficient to guarantee convergence (see Section \ref{sec:algorithm}.

   In combination with \refeq{eq:elbon} (we omit the first term which is independent of $\bpsi)$, this yields the following Monte Carlo approximation to the ELBO:
%Thus, equation (\ref{eq:elbon}) can now be written as
\be
\begin{array}{ll}
 \mathcal{F} (\bpsi) &  \approx  -\lambda \frac{N}{M} \sum_{k=1}^M \left< |r_{w_{j_k}}(\by,\bx)| \right> _{q_{\bpsi}(\bx,\by)} + \left< \log \cfrac{p(\by |\bx) p(\bx) }{q_{\bpsi}(\bx,\by)}\right>_{q_{\bpsi}(\bx,\by)} ~\text{where } j_k \sim Cat\left(N,\frac{1}{N}\right)
%  & - \left< log \cfrac{q_{\bpsi}(\bx,\by)}{p_{\bt}(\by |\bx) p(\bx) } \right>_{q_{\bpsi}(\bx,\by)}, ~\text{where } j_k \sim Categorical\left(p=\frac{1}{N}\right)
\end{array}
\label{eq:elboRandomResidual}
\ee
We discuss in Section \ref{sec:algorithm} how gradients of $\mathcal{F}$ can be computed and used in order to carry out the ELBO maximization.



%and solving the problem involves only maximizing $\mathcal{F}_{\bpsi}$ by using Stochastic Gradient Acsent (SGA). Algorithm \ref{alg:RandomResidual} summarizes the respective procedure.




==> section2/6_approximatingDensityForm.tex <==
\subsection{Form of the Approximating Density $q_{\bpsi}$}
\label{sec:ApproximatingDensity}

%\mc{Until we finalize the form of the covariance matrix I will use this simplified version. As soon as we have obtained good results for the covariance matrix that depends on $\bs{X}$ I will modify the following accordingly.}

In selecting the form of $q_{\bpsi}$ and without loss of generality  we postulate: 
\be
q_{\bpsi}(\bx,\by) = q_{\bpsi}(\by|\bx) q(\bx) = q_{\bpsi}(\by|\bx) p(\bx) %= \mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \boldsymbol{\Sigma}_{\bpsi})~\mathcal{N}\left(\bx | \bs{0}, \bs{I_{d_{\by}}}\right)
\label{eq:AppoxPostForm}
\ee 
i.e. we use the given density of the parametric input and attempt to approximate the input-to-output map with $q_{\bpsi}(\by|\bx)$ where $\bpsi$ denotes the tunable parameters. We note that alternate decompositions might be advisable in the context of inverse problems but are not discussed in this work.
We note also  that a deterministic formulation can be readily adopted by selecting a degenerate density in the form of a Dirac-delta, i.e.:
\be
q_{\bpsi}(\by|\bx)=\delta(\by-\bs{\mu}_{\bpsi} (\bx))
\ee
The sought function $\bs{\mu}_{\bpsi} (\bx)$ in this case can take the form of {\em any }
 of the proposed NN-based architectures such as Fully Connected Neural Networks (FCNNs), Convolutional Neural Networks (CNNs) \cite{zhu2019physics}, Deep Neural Operators (DeepONets) \cite{lu2019deeponet}, Graph Neural Operators (GNOs) \cite{li2020neural} or Fourier Neural Operators (FNOs) \cite{kovachki2021neural}, in which case $\bpsi$ would correspond to the associated NN-parameters.


While all these architectures have produced good results in a variety of problems, it is easily understood that as the variability and the dimension of the input $\bx$ (as well as of the sought output $\by$) increase, so must the complexity of the aforementioned NN-based schemes increase. At a practical level it is not uncommon that one must train for millions or billions of parameters $\bpsi$ (refs). This situation is much more pronounced in {\em multiscale} problems where input and output de facto require high-dimensional representations.


More importantly as such interpolators are agnostic of the physical context, they face significant problems in generalizing (refs). For example if out-of-distribution predictions are sought for a significantly different input $\bx$ as compared to the ones used in training, then the predictive accuracy can significantly drop (refs). In addition and in the context of PDEs in particular, if one were to seek predictions under a different set of boundary conditions than the ones employed during training, most likely, these predictions would be significantly off and by a large margin (see Section \ref{sec:numerical}). 

One could claim that enlarged datasets, or  bigger models or progress in pertinent hardware could alleviate or overcome these difficulties. Nevertheless none of these strategies address the fundamental underlying question which is how to find the requisite information bottlenecks that lead to  drastic dimensionality reductions and lightweight surrogates
 and how to achieve this in a problem-aware manner that is capable of producing accurate  predictions under extrapolative settings \cite{grigo_physics-aware_2019}.



%Given the high-dimensional setting, selecting an appropriate $q_{\bpsi}$ poses significant challenges as this needs to be simultaneously:
%\bi 
%\item \textbf{accurate}, i.e. it should envelop the true $\by$ for each $\bx$ and with the lowest possible uncertainty,
%\item \textbf{generalizable}, i.e. it should be capable of producing accurate predictions for inputs $\bx$ {\em not seen} during training as well as potentially for different boundary conditions or right-hand sides of the governing PDE, and
%\item \textbf{lightweight}, i.e. with a number of parameters $\bpsi$ that, at a minimum, does not grow rapidly with the dimension of the problem.
%\ei 
In view of these objectives and following previous work \cite{grigo_physics-aware_2019,rixner2021probabilistic}, we propose incorporating coarse-grained versions of the governing PDE as an implicit solver \cite{belbute2020combining,um2020solver} in the surrogate constructed. 
We  elaborate on this in the subsequent sections and more importantly we extend this {\em multiscale} problems which pose a unique set of challenges. 
%as previous works has shown, it is advisable  to incorporate as much as possible of the physical structure in $q_{\bpsi}$.
%, we incorporate a coarse-grained version of the reference, fine-grained model. We note that implicit solvers have also been employed in the past as e.g. in \cite{belbute2020combining,um2020solver}.  
For the purposes of the Variational Inference proposed, we employ a multivariate Gaussian of the form:
\be
q_{\bpsi}(\by|\bx)  = \mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \boldsymbol{\Sigma}_{\bpsi})
\label{eq:FormofTheAproxPosterior}
\ee
the mean and covariance of which are discussed in the sequel.
%where $\bs{\mu}_{\bpsi} (\bx)$ is the trainable mean prediction and $\boldsymbol{\Sigma}_{\bpsi}$ is a trainable covariance matrix. From equation \ref{eq:AppoxPostForm}, one can observe that only the mean prediction depends on the inputs. Moreover, the only trainable part of the approximate posterior is the conditional distribution $q_{\bpsi}(\by|\bx)$, which will be ultimately be used for making predictions after training the model. The form of the previous distribution is assumed to be Gaussian, and its parameters are described below. 

\psk{If covariance is described later then there is no reason to have a subsection here}
\subsubsection{Mean function $\bs{\mu}_{\bpsi} (\bx)$}
\label{sec:ApproximatingDensityMu}

In the context of  materials problems and as in the model formulation  of \refeq{eq:DarcyFlowEquation} where the inputs $\bx$ parametrize a, potentially multiscale, material property field,  we consider a (much) coarser, discretized version (see e.g. Figure \ref{fig:CGPhysicsArchitecture}) of the governing PDE where $\bxx, \byy$ denote the respective, discretized input and output. 
By construction, their dimension is much lower as compared to  their reference, fine-grained counterparts $\bx,\by$. As such, the solution of the associated (non)linear algebraic equations to obtain the solution $\byy$ for any input $\bxx$  is much faster.
As we have shown in \cite{grigo_physics-aware_2019}, the $\bxx$ could be thought of as some effective material properties  which serve as the requisite information bottleneck to the  problem. Furthermore, it is possible that  a different (discretized) PDE  could be used as a stencil for the coarse-grained model.
%on the coarse grid. In \cite{grigo_physics-aware_2019} we have shown that even a different PDE could be used as a stencil for the coarse-grained model.

We complement the implicit, differentiable, and vectorized, input-output map  $\byy(\bxx)$  of the CG model, with two additional components:
\bi
\item a fine-to-coarse input map denoted by $\bxx_{\bpsi}(\bx)$ that we express with a shallow CNN parametrized by $\bpsi$ (details in \ref{appendix:shallowCNN}) \psk{Please describe the general structure},
\item a coarse-to-fine output map denoted by $\by(\byy)$ that  attempts to reconstruct the reference, FG output $\by$ given the CG output $\byy$ ( details in \ref{appendix:ytoYTransform}) \psk{Please describe the general architecture}.
\ei
The composition of these three functions, i.e.:
\be
\bs{\mu}_{\bpsi} (\bx)=\by\left( \byy\left(\bxx_{\bpsi}(\bx) \right) \right)
\label{eq:formOfmeanPrediction}
\ee
In the formulation employed in the ensuing numerical experiments, the sole trainable parameters are associated with the inner layer i.e. the fine-to-coarse map from $\bx$ to $\bxx$. More complex formulations involving trainable parameters in the other two layers could be readily accommodated.

We note that all three layers are differentiable, and each evaluation requires a solution of the CG model. Differentiation of $\bs{\mu}_{\bpsi}$ with respect to $\bpsi$ as needed for training requires a backward pass which can be computed with Automatic Differentiation (refs) and/or adjoint formulations of the governing equations of the CG model (Refs).
%for obtaining derivatives.  
The advantages of the adopted model in view of the aforementioned desiderata  will become apparent in the numerical illustrations.


%This term has a particular coarse-grained, physics-retaining form, as shown in figure \ref{fig:CGPhysicsArchitecture}. The coarse-grained (CG) form of $\bs{\mu}_{\bpsi} (\bx)$ is

%\be
%\bx \xrightarrow{f_{\bpsi}(\cdot)} \bs{X} \xrightarrow{G(\cdot)} \bs{Y} \xrightarrow{h(\cdot)} \bs{\mu}_{\bpsi} (\bx)
%\ee
%
%where $f_{\bpsi}(\cdot)$ is a shallow CNN (more details in \ref{appendix:shallowCNN}, responsible for downsampling $\bx$ and learning the most relevant effective properties of $\bx$. After applying $f_{\bpsi}(\cdot)$ a low dimensional representation $\bs{X}$ of the inputs will be used in a fully vectorized and differentiable FEM solver $G(\cdot)$ to find a low dimensional representation of the mean outputs $\bs{Y}$. Lastly, a fixed linear map $h(\cdot)$ is used for acquiring the mean prediction $\bs{\mu}_{\bpsi} (\bx)$ (more details about $h(\cdot)$ in \ref{appendix:ytoYTransform}). The previous architecture allows faster convergence and more precise out-of-distribution predictions, where many state-of-the-art schemes collapse. Furthermore, with very few parameters, it can provide predictions of similar accuracy with state-of-the-art methods while providing uncertainty quantification.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.8\textwidth]{figs/Methodology/physicsSchematicWithMesh.png}
  \caption{Schematic illustration of the proposed, physics-aware procedure for parametrizing the mean solution $\bs{\mu}_{\bpsi} (\bx)$, given an input $\bx$ as described in subsection \ref{sec:ApproximatingDensityMu}. 
  %\psk{It would be good if the meshes good be shown to illustrate the difference in dimension} \mc{Does something like the above suffices?}
  }
  \label{fig:CGPhysicsArchitecture}
\end{figure}

%\psk{Given the different form adopted in 2.8 maybe this can be specialized in the num. illustrations to avoid confusion}
 



==> section2/7_CGLearning.tex <==
\subsection{Learning solutions to multiscale PDEs}
\label{sec:CGLearning}

As mentioned in section \ref{sec:proposedFramework}, an interesting case in which physics-informed methods struggle is when the solution has multiscale features. In many such situations, it would be sufficient to capture only the coarse-scale (low wavenumber - high wavelength) characteristics during the prediction phase of the surrogate. To our knowledge, there isn't currently any framework that has effectively addressed this issue. In our effort to solve this problem, we decompose the solution-output $\by$ as $\by=(\by_c, \by_f)$, where $\by_c$ accounts for the coarse-scale features we are interested in and $\by_f$ for the fine-scale fluctuations that are not of interest.

When labeled data, i.e. pairs of $\bx$ and $\by$ are available, it has been demonstrated \cite{zhang_gfinns_2021,hernandez2022thermodynamics,masi2022multiscale,cueto2023thermodynamics}, that predictive models for $\by_c$ can be learned.  On the contrary, when residuals (of any type) are used for training such models, it is necessary to consider both $\by_c$ and $\by_f$ as assuming the latter are zero or negligible can lead to big errors (refs. needed). As the dimension of $\by_f$ is in general much larger than that of $\by_c$ constructing models that account for its dependence on the input $\bx$ poses significant challenges and could require a lot of training data. 
%high-dimensional Unfortunately, in order to learn the input-output map, the framework needs to have access to a relatively large number of inputs during training. Consequently, the number of $\by_f$ high dimensional vectors to be learned would be large too, making training computationally very expensive or even infeasible.

In the context of the probabilistic models advocated, such a a task would entail learning $q_{\bpsi}(\by_f|\bx)$, and  $q_{\bpsi}(\by_c|\bx)$. We propose neglecting the dependence of $\bx$ on $\by_f$ in our model, without neglecting the effect of $\by_f$ in the residual. Thus, we propose to train the surrogate only by using a small fixed number of inputs, to keep the number of $\by_f$ and consequently the number of trainable parameters low. One needs to keep in mind, that this is possible only because of the physics-inspired architecture described in subsection \ref{sec:ApproximatingDensityMu}. This acts as an efficient informational bottleneck, which makes the surrogate easier to saturate, i.e. fewer input instances are needed for training.

To apply formally the above idea, we consider a reduced case where the density of the inputs $\bx$, can be approximated by $K$ instances each with a different probability $p_k$ as:

\begin{equation}
p(\bx) = \sum_{k=1}^K p_k \delta(\bx - \bx_k).
\end{equation}

\noindent As before we have the virtual observables $\hat{\mathbf{R}} = 0$ associated with the residuals $\{r_j(\by_c, \by_f, \bx)\}_{j=1}^N$ in the virtual likelihood $p(\hat{\mathbf{R}} | \by_c, \by_f, \bx)$. Given a prior $p(\by | \bx)$ as before, the corresponding ELBO will be the same as in equation \ref{eq:elbon}, with the only difference being:

\begin{equation}
    q_{\bpsi}(\bx, \by) = q_{\bpsi} (\by_c | \bx) q_{\bpsi}(\by_f | \bx_k) p(\bx)
\end{equation}

where $q_{\bpsi} (\by_c | \bx)$ has the same form as in equation \ref{eq:AppoxPostForm} and $q_{\bpsi}(\by_f | \bx_k)= \delta(\by_f - \by_{f,k})$. As a result, the only extra trainable parameters introduced in the above setup are $\by_{f,k}$, the dimension of which is equal to $K\cdot d_f$ (computationally manageable). After training, the density $q_{\bpsi}(\by_c | \bx)$ can be readily used for predictive purposes in very challenging multiscale setups, where the framework described in the previous chapters as well as other state-of-the-art physics-informed surrogates completely fail to learn the map from the inputs to the coarse-grained solution.

==> section2/8_tempering.tex <==
\subsection{Tempering of the hyperparameter $\lambda$}
\label{sec:algorithm}

\psk{This paragraph sounds very ad-hoc and suggests that you can select the solution you want at the end without any guiding principle. I suggest you move it after 2.6 and put it as part of a larger section on Algorithmic implementation. 
Therein it should be discussed how SVI is done (i.e. reparametrization trick + MC estimates of the gradient + stochastic gradient ascent) with appropriate references and very technical details moved to an appendix. Tempering could be a part of the overall scheme but it should be motivated appropriately  and a criterion should be defined of when u move to the next lambda.
I.e. algorithm 1 should be included and expanded}.
}
As discussed in \ref{infusingVirtualObservables}, the hyperparameter $\lambda$ controls how strongly the virtual observables will be enforced. This in turn, controls how wide will be the uncertainty bounds of the probabilistic predictions of the trained model. Thus, the selection of $\lambda$ is ultimately selected by the user of the algorithm, according to the respective objectives. Ultimately, the optimal $\lambda$ is different for each case it is up to the user to run a short calibration process to determine what $\lambda$ will result in the best suited for the problem uncertainty bounds range.




==> section2/9_Algorithm.tex <==
\begin{algorithm}[H]
% \caption{Simple Description of the Learning Algorithm.}
\begin{algorithmic}[1]
    \State  $\bpsi\gets \boldsymbol{\psi_0}$; \Comment{Initialization of $\boldsymbol{\psi}$}
\While{$\mathcal{F}_{\bpsi}$ not converged} 
   \State $k \sim Categorical\left(p=\frac{1}{N}\right)$; \Comment{Drawing random $k$}
   \State  $\bx_{m}, ~ \by_{m} \sim q_{\boldsymbol{\psi}}(\bx, \by), ~~~~ m = 1, 2, ..., M$ 
   \State Estimate $\nabla_{\bpsi} \mathcal{F}_{\bpsi}$ \Comment{
    %\gets \frac{1}{M}\sum_{n_m=1}^{N_m}\hat{\mathcal{F}}(q_{\bpsi}(\bx_{n_m},\by_{n_m}), \hat{\boldsymbol{\phi}}_{max})$ // 
    \textbf{Monte Carlo} estimate of $\nabla_{\bpsi} \mathcal{F}_{\bpsi}$  with \textbf{Reparameterization trick}} %estimate of $\hat{\mathcal{F}}$
    \State $\bpsi_{\ell+1} \gets \bpsi_{\ell} + \boldsymbol{\rho}^{(\ell)} \odot \nabla_{\bpsi} \mathcal{F}_{\bpsi}$ \Comment{ \textbf{SGA  using ADAM} }
    \State $\ell \gets \ell + 1$
\EndWhile
\end{algorithmic}
\caption{Random Residual Algorithm.}
%\caption{Assuming $q_{\bpsi}(\bx,\by)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T)~\mathcal{N}\left(\bx | \bs{0}, \bs{I}\right)$ }
\label{alg:RandomResidual}
%\psk{Algorithms should come after the full model has been presented}
\end{algorithm}

==> section2/greedyAlgorithm.tex <==
\subsection{Greedy Algorithm}
\label{sec:GreedyAlgorithm}

Another approach is to obtain a virtual observable dataset $\boldsymbol{R}_N(\bx, \by) = \{r_{w_j}(\bx, \by)\}_{j=1}^N$ of higher informational content than a random choice, while keeping equation (\ref{eq:elbon}) intact. The idea is to start with zero residuals $r_{w_j}(\bx, \by)$ in which case $q_0$ is the prior and successively add one residual at a time (i.e. selecting a new $w$ or $\bphi$) based on maximizing the KL-divergence between the theoretical posterior which is based on $n$ and the one based on $n+1$ virtual observables, i.e. $KL\left( p_n || p_{n+1} \right)$. Given the unavailability of $p_n$, we consider $H(\bphi) = KL\left(q_n || p_{n+1}\right)$ as our objective function for finding the best new virtual observable to add next, since $q_n$ encapsulates our knowledge about the problem after $n$ steps. The fine details for the estimation of the above loss function $H(\bphi)$ and the respective gradients can be found in \ref{appendix:HEstimation}.

Having access to estimates of the gradients of $H(\bphi)$ the iterative algorithm \ref{alg:Greedy} can be formulated, where SVI is performed each time until convergence of the ELBO by using $n$ virtual observables, before finding the best new $(n+1)_{th}$ observable to add to the posterior by using SGD.

\begin{algorithm}[H]
% \caption{Simple Description of the Learning Algorithm.}
\begin{algorithmic}[1]
    \State $\boldsymbol{\phi} \gets \boldsymbol{\phi_0}$; $\bpsi\gets \boldsymbol{\psi_0}$; // Initialization  $\boldsymbol{\phi}$ and $\boldsymbol{\psi}$
\While{$\Delta H > \epsilon $}
\For{n = 1, N} 
    \For{$k \gets 1, K$} // Searching the best new $w_{N+1}$ to add
       \State  $\bx_{m}, ~ \by_{m} \sim q_{\boldsymbol{\psi}}(\bx, \by), ~~~~ m = 1, 2, ..., M$ 
       \State Estimate: $\nabla_{\bphi} H$  // Using the method described in \ref{appendix:HEstimation}
       \State $\boldsymbol{\phi}_{k+1} \gets \boldsymbol{\phi}_k - \boldsymbol{\rho}_{\bphi}^{(k)} \odot \nabla_{\bphi}H $ // \textbf{SGD using ADAM}
      \State \textbf{return} $\bphi_n \gets \boldsymbol{\phi}_K$
    \EndFor  
    \For{$\ell \gets 1, L$} // Maximization of the ELBO w.r.t. $\boldsymbol{\psi}$ (\textbf{SVI})
%     \State Sample $\bx_m \sim p(\bx), \boldsymbol{\epsilon}_{m} \sim \mathcal{N}\left(0, I\right), ~~~~ m = 1, 2, ..., M$ // \textbf{Reparameterization trick} %(if MVNs are used)
%     \State %$\bx_{m} \gets \mathbf{m}_{\bx} + \mathbf{L}_{\bx} \odot \boldsymbol{\epsilon}_{n_m}, ~~~ 
%     $\by_{m} \gets \mathbf{m}_{\bpsi}(\bx_{m}) + \mathbf{V}_{\bpsi}(\bx_{m}) \odot \boldsymbol{\epsilon}_{m} , ~~~~ m = 1, 2, ..., M$
    \State Estimate $\nabla_{\bpsi} \mathcal{F}_{n, \bpsi}$ // 
    %\gets \frac{1}{M}\sum_{n_m=1}^{N_m}\hat{\mathcal{F}}(q_{\bpsi}(\bx_{n_m},\by_{n_m}), \hat{\boldsymbol{\phi}}_{max})$ // 
    \textbf{Monte Carlo} of $\nabla_{\bpsi} \mathcal{F}_{n, \bpsi}$  with \textbf{Reparameterization trick} %estimate of $\hat{\mathcal{F}}$
     \State $\bpsi_{\ell+1} \gets \bpsi_{\ell} + \boldsymbol{\rho}_{\bpsi}^{(\ell)} \odot \nabla_{\bpsi} \mathcal{F}_{n, \bpsi}$// \textbf{SGA  using ADAM}
    \State \textbf{return} $\bpsi \gets \boldsymbol{\psi}_L$
    \EndFor
\EndFor
\EndWhile
\end{algorithmic}
\caption{Greedy Algorithm.}
%\caption{Assuming $q_{\bpsi}(\bx,\by)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T)~\mathcal{N}\left(\bx | \bs{0}, \bs{I}\right)$}
\label{alg:Greedy}
\end{algorithm}

==> section2/saddlePointAlgorithm.tex <==
\psk{Unless 2.5 and 2.6 are  used in any of the num. illustrations, please skip the detailed discussion and just make a short remark about these possibilities referring to future work}.  


\subsection{Saddle Point Algorithm}
 If the weight functions are parameterized by using some parameters $\bphi$, then the most penalizing and thus informative residuals would be the ones that maximize the expected squared residual for a given variational distribution $q_{\bpsi}(\bx,\by)$

\be
\bphi_{\bpsi} =\arg \max_{\bphi} \mathbb{E}_{q_{\bpsi}(\bx,\by)} \left[ r^2_{w_{\bphi}} (\bx,\by) \right]
\ee

the additional constraint $|\bphi|^2=1$ should be introduced to maintain the norm of $\bphi$ finite as the number of iterations of any maximization scheme increases. The selection of the most informative weight function allows to further lower-bound the ELBO from equation (\ref{eq:elbon})

\be
\begin{array}{ll}
\log p( \hat{\bs{R}}) \ge \mathcal{F}_{\bpsi} & = -\frac{\lambda}{2} \sum_{j=1}^N \left< r_{w_j}^2(\by,\bx) \right> _{q_{\bpsi}(\bx,\by)}
  - \left< log \cfrac{q_{\bpsi}(\bx,\by)}{p_{\bt}(\by |\bx) p(\bx) } \right>_{q_{\bpsi}(\bx,\by)} \\
& \ge -\frac{N \lambda}{2} \left< r_{w_{\bphi_{\bpsi}}}^2(\by,\bx) \right> _{q_{\bpsi}(\bx,\by)} - \left< log \cfrac{q_{\bpsi}(\bx,\by)}{p_{\bt}(\by |\bx) p(\bx) } \right>_{q_{\bpsi}(\bx,\by)} \\
& = min_{\bphi} \mathcal{F}_{\bpsi, \bphi}
\end{array}
\ee


An algorithmic scheme can be derived from the equations mentioned earlier to find the approximate posterior. The scheme will involve the iterative maximization of the ELBO w.r.t the parameters $\bpsi$ followed by a minimization of the ELBO w.r.t. the parameters $\bphi$ for every optimization cycle. Therefore, a saddle point optimization problem must be solved before obtaining the approximate posterior. The steps of the algorithm are outlined in algorithm \ref{alg:SaddlePoint}, where Stochastic Gradient Descent/Ascent is employed for the update of $\bphi$/$\bpsi$ by using the \textit{ADAM} \cite{kingma2014adam} optimizer for adapting the learning rates. In figure \ref{fig:ELBO_lower_bound}, the decisive contribution of the minimization loop of algorithm \ref{alg:SaddlePoint} is illustrated.

%%% The algorithm has some bugs
\begin{algorithm}[H]
% \caption{Simple Description of the Learning Algorithm.}
\begin{algorithmic}[1]
    \State $\boldsymbol{\phi} \gets \boldsymbol{\phi_0}$; $\bpsi\gets \boldsymbol{\psi_0}$; // Initialization  $\boldsymbol{\phi}$ and $\boldsymbol{\psi}$
\While{$||\frac{\partial \mathcal{F}_{\bpsi, \bphi}}{\partial ( \boldsymbol{\psi}, \boldsymbol{\phi})}|| > \varepsilon$ } 
    \For{$k \gets 1, K$} // Minimization of $\mathcal{F}_{\bpsi, \bphi}$ w.r.t. $\boldsymbol{\phi}$
       \State  $\bx_{m}, ~ \by_{m} \sim q_{\boldsymbol{\psi}}(\bx, \by), ~~~~ m = 1, 2, ..., M$ 
       \State Estimate: $\nabla_{\bphi} \mathcal{F}_{\bpsi, \bphi} \gets 
       -\frac{1}{M} \sum_{m=1}^{M} \nabla_{\bphi} r_{w_{\boldsymbol{\phi}}}^2(\bx_{m},\by_{m})$ // \textbf{Monte Carlo} estimate of $\nabla_{\bphi} \mathcal{F}_{\bpsi, \bphi}$ %of $< r_{w_{\boldsymbol{\phi}_k}}^2(\by,\bx)>_{q_{\bpsi}(\bx,\by)}$
       \State $\boldsymbol{\phi}_{k+1} \gets \boldsymbol{\phi}_k - \boldsymbol{\rho}_{\bphi}^{(k)} \odot \nabla_{\bphi} \mathcal{F}_{\bpsi, \bphi} $ // \textbf{SGD using ADAM}
      \State \textbf{return} $\bphi_{\bpsi} \gets \boldsymbol{\phi}_K$
    \EndFor  
    \For{$\ell \gets 1, L$} // Maximization of the ELBO w.r.t. $\boldsymbol{\psi}$ (\textbf{SVI})
%     \State Sample $\bx_m \sim p(\bx), \boldsymbol{\epsilon}_{m} \sim \mathcal{N}\left(0, I\right), ~~~~ m = 1, 2, ..., M$ // \textbf{Reparameterization trick} %(if MVNs are used)
%     \State %$\bx_{m} \gets \mathbf{m}_{\bx} + \mathbf{L}_{\bx} \odot \boldsymbol{\epsilon}_{n_m}, ~~~ 
%     $\by_{m} \gets \mathbf{m}_{\bpsi}(\bx_{m}) + \mathbf{V}_{\bpsi}(\bx_{m}) \odot \boldsymbol{\epsilon}_{m} , ~~~~ m = 1, 2, ..., M$
    \State Estimate $\nabla_{\bpsi} \mathcal{F}_{\bpsi, \bphi}$ // 
    %\gets \frac{1}{M}\sum_{n_m=1}^{N_m}\hat{\mathcal{F}}(q_{\bpsi}(\bx_{n_m},\by_{n_m}), \hat{\boldsymbol{\phi}}_{max})$ // 
    \textbf{Monte Carlo} of $\nabla_{\bpsi} \mathcal{F}_{\bpsi, \bphi}$  with \textbf{Reparameterization trick} %estimate of $\hat{\mathcal{F}}$
     \State $\bpsi_{\ell+1} \gets \bpsi_{\ell} + \boldsymbol{\rho}_{\bpsi}^{(\ell)} \odot \nabla_{\bpsi} \mathcal{F}_{\bpsi, \bphi}$// \textbf{SGA  using ADAM}
    \State \textbf{return} $\bpsi \gets \boldsymbol{\psi}_L$
    \EndFor
\EndWhile
\end{algorithmic}
\caption{Saddle Point Algorithm.}
%\caption{Assuming $q_{\bpsi}(\bx,\by)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T)~\mathcal{N}\left(\bx | \bs{0}, \bs{I}\right)$}
\label{alg:SaddlePoint}
\end{algorithm}

\begin{figure}[H]\centering
\def\svgwidth{0.8\textwidth}
\import{figs/}{ELBO.eps_tex}
\caption{Visualization of the gradual evolution of the ELBO lower bound. For a given parameter $\bpsi$, as the iterations of the 1st optimization loop in figure \ref{alg:SaddlePoint} proceed, gradually improved approximations (lower-bounds) of the ELBO are produced.}
\label{fig:ELBO_lower_bound}
\end{figure}

==> section2/section2.tex <==
\section{Methodology}

%\psk{if $\by$ is a vector, $\mathcal{L}$ cannot be a differential operator. You need to distinguish between the continuous version (strong form) and the discretized. The latter can come after you introduce the weighted residuals. You have do be careful in defining densities on function spaces, see e.g. \cite{alberts_physics-informed_2023,
%chen_solving_2021}} \mc{Thank you for the comment. I tried to create a more solid definition. Do you think that this is now solid or do I need to correct it further?}

We are concerned with parametrized PDEs which can be generally written as:
%The general problem for which the framework will be developed, is described in the following equations:


\be
\begin{array}{ll}
\mathcal{L}(c(\bs{s,x}), u(\bs{s}))=0,~~~ \bs{s} \in \Omega & \textrm{((non)linear differential operator)} \\
\mathcal{B}(c(\bs{s,x}), u(\bs{s}))=0, \quad \bs{s} \in \pa \Omega & \textrm{(boundary-conditions  operator)} \\
\end{array}
\ee
%
where $\bs{s}$ denotes space, $\Omega \subset \RR^{d_s}$ the problem domain,  $c(\bs{s,x})$ denotes an input function parametrized  by $\bx \in \mathcal{X} \subset \RR^{d_x}$ (e.g. material property field) and  $u(\bs{s})$ the sought solution to the boundary value problem above. 
In the following we adopt a discretized representation of the solution i.e. $u(\bs{s})\xrightarrow[]{\text{discretize}} \by$ where $\by \in \mathcal{Y} \subset \RR^{d_y}$. We assume that that the adopted discretization is fine enough to provide an acceptable approximation to the actual solution which in general implies that $dim(\by)>>1$. The vector $\by$ could represent coefficients with respect to a given set of functions (e.g. FE shape functions, Radial Basis Functions,  Fourier, Wavelet) or the weight/biases of a  neural network.  We adopt a finite-dimensional, albeit potentially high-dimensional, representation of the input and output although this can be relaxed +++++++\cite{fanaskov_spectral_2023}.



% \in \mathcal{Y}$ is the unknown/solution function of the parametric PDE. We denote with $c(\bs{s}, \bx)$ and $u(\bs{s}, \by)$ some discretized versions of $c(\bs{s})$ and $u(\bs{s})$ respectively, where $\bx$ is the input vector $\bx \in R^{d_{\bx}}$ and $\by$ the output/unknown vector $\by \in R^{d_{\by}}$. 

We aim at  developing a {\em probabilistic} surrogate which will be expressed in the form of a density $q(\by |\bx)$ that can predict the (discretized) solution for any input $\bx$ and especially in the high-dimensional setting i.e. when $d_x,d_y>>1$.
We note that the predictive uncertainty in this case is not due to aleatoric stochasticity in the governing equations (although such cases can be accommodated as well) but of epistemic nature due to the use of partial, and hopefully small, data in constructing this surrogate as explained in the sequel. 
%
%In most cases of practical interest, the dimensions of the inputs and outputs are high, i.e. $d_{\bx}, ~d_{\by} >> 1$, and the times that the above equations need to be inquired are high as well (e.g. optimization under uncertainty or forward/inverse uncertainty quantification problems). The goal of the proposed framework is to train an approximate predictive surrogate $q(\by| \bx)( \bs{s})$, which will be capable of providing computationally inexpensive probabilistic predictions about $\by$ for any given $\bx$ at the requested spatial coordinates $\bs{s}$. In other words, we attempt to learn an approximation of the map $\mathcal{X} \rightarrow \mathcal{Y}$ between the functions $c(\bs{s})$ and $u(\bs{s})$.



\subsection{Strong and Weak of a boundary-value problem}
\label{sec:SWform}

We view the governing PDE as an infinite source of information which we probe with the help of {\em weighted residuals}. These constitute the (virtual) data with which we attempt to train our surrogate.
In order to illustrate this concretely and clearly, we use as an example a linear, elliptic PDE. The methodological elements can then be generalized to other types of PDEs.
In particular, we consider the boundary value problem:
%For the derivation of the framework, the strong form of the parametric PDE should be firstly written. As an example, we will use a simple parametric Elliptic PDE with its respective boundary conditions 

\be
\begin{array}{rl}
 \nabla (-c(\bs{s}, \bx) \nabla u(\bs{s}))=g, & \bs{s} \in \Omega\\
 u(\bs{s})=u_0, &   \bs{s} \in \Gamma_u \\
 -c(\bs{s}, \bx) \nabla u(\bs{s}) \bs{n}=q_0, &  \bs{s} \in \Gamma_q =\pa \Omega - \Gamma_u
\end{array}
\label{eq:DarcyFlowEquation}
\ee
%\psk{$\by$ are not parameters that $u$ depends on but the representation of $u$ upon discretization}
where $c(\bs{s}, \bx)$ is a (random) conductivity/permeability/diffusivity  field which depends on the parameters $\bx$. %, % $g$ is the term of the external forces applied, $u(\bs{s})$ is the solution field, $\Omega$ is the definition space, 
We denote with $\Gamma_u$ and $\Gamma_q$ the parts of the boundary  where Dirichlet and Neumann conditions are respectively defined. The symbol $\bs{n}$ indicates the outward vector, which is normal to the boundary, while the $u_0$ and $q_0$ denote the prescribed values. % of at the boundaries, where Dirichlet and Neumann conditions are respectively applied.

We employ candidate solutions $u_{\by}$ which are represented by the finite-dimensional  $\by \in \RR^{d_y}$ as discussed above and which are assumed to a priori satisfy the Dirichlet BCs \footnote{This requirement is consistent with traditional derivations but can be readily relaxed or removed in our formulation.}. These are combined with weighting functions $w(\bs{s}) \in \mathcal{W}$ which are assumed to be zero at the Dirichlet boundary i.e. $w(\bs{s})|_{\bs{s} \in \Gamma_u}=0$.
%For the solution field $u(\bs{s})$ we select the following representation:
%
%\be
%u(\bs{s})=\sum_{j=1}^n y_j \phi_j(\bs{s}),
%\label{eq:trialSolRepresentation}
%\ee

%\noindent where $\bs{y}$ are the output vector (coefficients of the solution representation), $n=dim(\by)$ and $\phi_j(\bs{s})$, are the corresponding shape/basis functions. If $w$ denotes appropriate weight functions such that $w(\bs{s})|_{\bs{s} \in \Gamma_u}=0$, then the weak form of the above equation will be \cite{finlayson_method_1972}
By employing integration-by-parts \cite{finlayson_method_1972} and for each such $w(\bs{s})$ we obtain the weighted residual:
\be
r_w(\by,\bx) = 0= \int_{\Gamma_q} w~ q_0 ~d\Gamma+\int_{\Omega} \nabla w~ c(\bs{s}, \bx) ~\nabla u_{\by}~ d\bs{s} -\int_{\Omega} w~ g ~d\bs{s}.
\label{eq:weak1}
\ee

\noindent We note that depending on the choice of the weight functions $w$ (at least) six methods (i.e. collocation, sub-domain, least-squares, (Petrov)-Galerkin, moments) arise as  special cases \citep{finlayson_method_1972}. As it will become apparent in the sequel, the weighted residuals are used as data sources and not in  the traditional sense, i.e. to derive a discretized system of equations  for the approximate solution of the problem. Hence we would be at liberty to consider alternate or even non-symmetric versions with respect to $u$ and $w$ as for example by applying  further integration-by-parts which would  lead to expressions with  lower-order derivatives of the candidate solution $u_{\by}$.

%\psk{
%\noindent \textbf{Remarks:}
%\begin{itemize}
%\item Depending on the choice of the weight functions $w$ (at least) six methods (i.e. collocation, sub-%domain, least-squares, (Petrov)-Galerkin, moments) arise as  special cases \citep{finlayson_method_1972}.
%\item Since weighted residuals are not employed here in the traditional sense and in order to obtain %approximate solutions to the PDE, we are at liberty to consider alternative versions. For example, it is %not necessary that the final form is symmetric with respect to $u$ and $w$ but integration-by-parts could %further be employed in order to obtain expressions that contain lower-order derivatives of the candidate %solution $u$. 
%\end{itemize} }



\subsection{ Virtual Observables and Virtual Likelihhod} \label{infusingVirtualObservables}

Rather than solving the governing equations multiple times for different values of $\bx$ in order to obtain a {\em labeled} training dataset (i.e. pairs of $(\bx,\by)$) %In the case of training with labeled data, the above PDE should be inquired many times for different inputs $\bx$ and spatial coordinates $\mathbf{s}$ in order to create the necessary pairs of data for the training. In our formulation, this process is completely avoided 
we treat weighted residuals as in \refeq{eq:weak1} as {\em virtual observables} \cite{kaltenbach2020incorporating}.
In particular, given   $N$ distinct weighting function $w_j$ and the corresponding residuals $r_{w_j}(\by,\bx)$, we consider that their values $\hat{r}_j$ have been {\em virtually} observed and are equal to $0$ i.e. the solution pairs $(\bx,\by)$ perfectly satisfy them. The {\em virtual} observables $\hat{\bs{R}}=\{ \hat{r}_j=0 \}_{j=1}^N$ imply a {\em virtual} likelihood which is assumed to be of the form: 
%are assumed to be equal to $0$ and relate to the  $r_{w_j}$ as follows:
%This is achieved by considering $N$ different weight functions $w_j$ and their corresponding residuals $r_{w_j}$. Thus, the training dataset will be given by the associated virtual observables $\hat{\bs{R}_N}=\{ \hat{r}_j=0 \}_{j=1}^N$. In other words, the residuals of the respective weight functions from equations (\ref{weak1}) are assumed to be equal to zero. The virtual data needs to be introduced to the probabilistic framework via the likelihood. Hence, the virtual observables are distorted with noise, as shown in the following equation

%\be
%0=\hat{r}_j=r_{w_j}(\by, \bx)+\frac{1}{\sqrt{\lambda}} \epsilon_r, \qquad \epsilon_r \sim p(\epsilon_r),
%\ee
%
%where $\lambda$ is the precision of the noise. Even though a Gaussian noise $\left( p(\epsilon_r)=\frac{1}{\sqrt{2 \pi}}exp{\left(-\frac{\epsilon_r^2}{2}\right)}\right) $ is most commonly used for constructing the likelihood, after experiments, it was concluded that a Laplacian noise $\left( p(\epsilon_r)=\frac{1}{2}exp\left(-|\epsilon_r|\right) \right)$ leads to faster training. This might be happening, because the partial derivatives $\frac{\partial r_{w_j}}{\partial \bx}$ or $\frac{\partial r_{w_j}}{\partial \by}$ are better behaved in the latter case. In turn this implies a {\em virtual} likelihood $p(\hat{\bs{R}} | \by, \bx)$\footnote{dependence on $\lambda$ is omitted} such that:
\be
\begin{array}{ll}
 p(\hat{\bs{R}} | \by, \bx) & =\prod_{j=1}^N p(\hat{r}_j=0 | \by, \bx) \\
 & = \prod_{j=1}^N \frac{\lambda}{2}  e^{ - \lambda |r_{w_j}(\by,\bx)|}
 %Laplace(\hat{r}_j=0 | r_{w_j}(\by, \bx), \lambda^{-1}) 
 \end{array}
\label{eq:virtuallike}
\ee
%
The role of the hyper-parameter $\lambda$ is significant as it controls how the likelihood of a pair $(\bx,\by)$ will decay if the corresponding residuals $r_{w_j}((\by, \bx)$ are different from zero. We note that alternative forms of the virtual likelihood are also possible (e.g. Gaussian)  but the form above was found to yield better results in the numerical experiments performed.  The role of the virtual observables/likelihood is to  provide information from the governing equations {\em without} having to solve them. We discuss in the sequel how this virtual likelihood can be used to learn a surrogate of the PDE solver and how this can be carried out by evaluating a few residuals at a time (i.e. without ever solving the weak form). 
%were carried out 
%On the other side, $r_{w_j}(\by, \bx)$ is the location parameter of the Laplacian distribution, obtained inexpensively by integrating numerically the equations (\ref{weak1}).



\subsection{Learning surrogates as probabilistic inference}
\label{sub:probInference}

Let $p(\bx)$ be a density on the parametric input. In the case of a random input this is directly furnished by the problem definition. For deterministic problems this could simply be a uniform density over the domain of possible values of $\bx$. 
We complement this with a {\em prior} density $p(\by|\bx)$. In the ensuing numerical experiments a vague, uninformative  such  prior was selected. We note that its role is not provide a good approximation of the sought output $\by$ given an input $\bx$ as this is to be achieved by  the {\em posterior} discussed later. Naturally though,  informative priors could accelerate inference. Parametrized versions could also be employed as e.g. in \cite{rixner2021probabilistic}  and the parameters can be fine-tuned as discussed in the the Remarks at the end of section \ref{sub:probInference} +++++.

The combination of the aforementioned prior densities with the virtual likelihood of \refeq{eq:virtuallike} in the context of  Bayes' rule leads to the {\em joint} posterior $p(\bx, \by | \hat{\bs{R}})$ as follows:
%After obtaining the likelihood, the posterior can be written by using Bayes Rule

\be
\begin{array}{ll}
p(\bx, \by | \hat{\bs{R}}) & =\cfrac{ p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx) }{ p(\hat{\bs{R}}) } \\
%& \propto p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx)  
\end{array}
\label{eq:postint}
\ee
We  emphasize the posterior above is defined on the {\em joint} space of inputs and outputs. Apart from the effect of the prior, it assigns highest probability to pairs of $\bx$ and $\by$ that achieve  $0$ residuals as is the case when they are a solution pair of the boundary value problem.

%where the term $p(\hat{\bs{R}})$ is the evidence and the term $p(\by |\bx) p(\bx)$ is a properly selected prior. The last could be just an uninformative prior in the simplest case, but if mildly parameterized, such a prior could significantly accelerate the convergence of the algorithm. For example, this prior could be a coarse-grained component of the scheme that quickly restricts the algorithm from exploring non-physical solutions.

Since the posterior is generally intractable, we advocate a Variational Inference scheme (refs) \mc{\cite{hoffman2013stochastic,paisley2012variational}?}
 i.e. we seek an approximation from a parametrized family of densities $q_{\bpsi}(\bx,\by)$ by minimizing the Kullback-Leibler divergence with the exact posterior above. 
 If $\bpsi$ denotes the tunable parameters, this is equivalent (refs) \mc{\cite{blei2017variational}?} to maximizing the Evidence Lower BOund (ELBO) $\mathcal{F}(\bpsi)$ to the log-evidence $\log p(\hat{\bs{R}})$ i.e.:
%The posterior could be approximated by using SVI \cite{paisley2012variational}, \cite{hoffman2013stochastic}. Starting from the Evidence, on can derive the ELBO as shown in the following equation:

\be
\begin{array}{ll}
 \log p( \hat{\bs{R}}) & = \log \int   p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx) ~d\by ~d\bx \\
 & \ge \left< \log \cfrac{   p( \hat{\bs{R}} | \bx, \by) p(\by |\bx) p(\bx) }{q_{\bpsi}(\bx,\by)} \right>_{q_{\bpsi}(\bx,\by)} \\
 & =\mathcal{F} (\bpsi) %= ELBO_{\bpsi}
 \end{array}
 \label{eq:logevi}
\ee
where the brackets $<.>_{q}$ indicate an expectation with respect to $q$. 
Substitution of \refeq{eq:virtuallike} 
 in the expression above leads to:
 %where variational approximation $q$ is trained by using the parameters $\bpsi$. Furthermore, equation \ref{eq:logevi} could be further expanded in the two following terms

\be
\begin{array}{ll}
 \mathcal{F} (\bpsi) &  = N\log \frac{\lambda}{2} - \lambda \sum_{j=1}^N \left< |r_{w_j}(\by,\bx)|\right> _{q_{\bpsi}(\bx,\by)}+ \left< \log \cfrac{p(\by |\bx) p(\bx) }{q_{\bpsi}(\bx,\by)}\right>_{q_{\bpsi}(\bx,\by)} \\
& = N\log \frac{\lambda}{2} - \lambda \sum_{j=1}^N \left< |r_{w_j}(\by,\bx)|\right> _{q_{\bpsi}(\bx,\by)}-KL\left(q_{\bpsi}(\bx,\by) ||  p(\by |\bx) p(\bx) \right) \\
 \end{array}
\label{eq:elbon}
\ee
Apart from the first term, which is irrelevant when $\bs{\lambda}$ is fixed, we note that the objective above promotes $q_{\bpsi}$ that simultaneously  minimize (on average) the absolute values of the $N$ residuals considered while minimizing the KL-divergence from the prior density adopted. 

\noindent \textbf{Remarks:}\\
\bi
\item The KL-divergence term in \refeq{eq:elbon} can be thought of  as a regularization or penalty term, which  nevertheless arises naturally in the Bayesian framework adopted.  In other physics-informed schemes that have been proposed (refs), ad-hoc parameters are generally selected as relative weights of these two terms. Similarly, alternative forms of virtual likelihoods  can give rise to the exact expressions found in competitive schemes. E.g. the use of a Gaussian likelihood would yield the sum of the {\em squares} of the $N$ residuals in the ELBO.
%
\item Furthermore such schemes generally employ collocation-type residuals in the physics-informed term \cite{raissi2019physics,lu2019deeponet,wang2021learning,li2021physics,nabian2018deep,zang2020weak}, which in our formulation arise as a special case  when the weight functions considered take the form of Dirac-deltas i.e. $w_j(\bs{s})=\delta(\bs{s}-\bs{s_j})$ where $\bs{s}_j$ correspond to the collocation points.
%
\item More importantly, by finding the optimal $q_{\bpsi}$ we obtain a {\em probabilistic surrogate} that is capable of providing probabilistic predictions of the solution $\by$ for any input $\bx$. Since the form of $q_{\bpsi}$ is critical to the accuracy of the proposed scheme we defer detailed discussions to Section \ref{sec:ApproximatingDensity}. As a final note we mention that if a degenerate $q_{\bpsi}$ is selected in the form of a Dirac-delta, then one obtains a {\em deterministic} surrogate as is the majority of the ones proposed in the literature \cite{raissi2019physics,lu2019deeponet,yu2018deep}. 
\ei
 



%To find the best possible approximate posterior $q_{\bpsi}(\bx,\by)$, both terms need to be minimized. The second one implies that the KL divergence of the approximate posterior from the prior needs to be minimized. The first term, on the other hand, states that the mean absolute value of the residuals should be minimized. In most physics-informed methods \cite{wang2021learning}, \cite{li2021physics}, the collocation method is used, which is a special case of the weighted residual method above. The form of the weight functions used in these cases is 

%\be
%w_j = \delta(\mathbf{s} - \mathbf{s}_j)
%\ee

%which has the property

%\be
%\int_{\Omega} r_j \delta(\mathbf{s} - \mathbf{s}_j) d\mathbf{s} = \left. r_j \right|_{\mathbf{s}_j}
%\ee


%After a second inspection of the first term, a question that naturally arises, is which and how many weight functions should be used to inquire the PDE as efficiently as possible. The following subsection describes a simple but efficient algorithm for doing so.


\subsection{Randomized Residual Algorithm}
\psk{Probably this should be discussed with the other algorithmic aspects as it is another MC approximation}
The evaluation and, more importantly,  the maximization of the ELBO $\mathcal{F}(\bpsi)$ requires the computation of the expectations with respect to $q_{\bpsi}$ of the absolute values of the $N$ weighted-residuals appearing in the virtual likelihood. We note that the evaluation of a weighted residual involves the computation of an integral over the problem domain (see e.g. \refeq{eq:weak1}) but not the solution of the PDE. These integrations can be carried out using deterministic or Monte-Carlo-based numerical integration schemes (refs). Furthermore if the weight functions have support on a subset of the problem domain $\Omega$ additional efficiencies can be achieved in the numerical integration. 


Independently of the particulars, it is readily understood that  as $N$ increases so does the information we extract from the governing PDE but so does also the computational effort. 
In order to improve the computational efficiency of these updates we propose a Monte Carlo approximation of the pertinent term in the ELBO in \refeq{eq:elbon}. In particular
%The sum, which appears in equation (\ref{eq:elbon}) can be approximated by Monte Carlo as follows

\begin{equation}
\sum_{j=1}^N \left< |r_{w_j}(\by,\bx)| \right> _{q_{\bpsi}(\bx,\by)} \approx \frac{N}{M} \sum_{k=1}^M \left< |r_{w_{j_k}}(\by,\bx)| \right> _{q_{\bpsi}(\bx,\by)}, ~\text{where } j_k \sim Cat\left(N,\frac{1}{N}\right)
\end{equation}
In essence, we sample at random and with equal probability $M<N$  weight functions out of the $N$ and use them to approximate the sum. As $M$ increases so does the Monte Carlo error decrease but so does the computational effort decrease. Since the Monte Carlo estimator is unbiased, even $M=1$ i.e. evaluating a single residual is sufficient to guarantee convergence (see Section \ref{sec:algorithm}.

   In combination with \refeq{eq:elbon} (we omit the first term which is independent of $\bpsi)$, this yields the following Monte Carlo approximation to the ELBO:
%Thus, equation (\ref{eq:elbon}) can now be written as
\be
\begin{array}{ll}
 \mathcal{F} (\bpsi) &  \approx  -\lambda \frac{N}{M} \sum_{k=1}^M \left< |r_{w_{j_k}}(\by,\bx)| \right> _{q_{\bpsi}(\bx,\by)} + \left< \log \cfrac{p(\by |\bx) p(\bx) }{q_{\bpsi}(\bx,\by)}\right>_{q_{\bpsi}(\bx,\by)} ~\text{where } j_k \sim Cat\left(N,\frac{1}{N}\right)
%  & - \left< log \cfrac{q_{\bpsi}(\bx,\by)}{p_{\bt}(\by |\bx) p(\bx) } \right>_{q_{\bpsi}(\bx,\by)}, ~\text{where } j_k \sim Categorical\left(p=\frac{1}{N}\right)
\end{array}
\label{eq:elboRandomResidual}
\ee
We discuss in Section ++++ how gradients of $\mathcal{F}$ can be computed and used in order to carry out the ELBO maximization.
\psk{Add short remarks alluding to more intelligent selection of weighting functions without technical details}
%and solving the problem involves only maximizing $\mathcal{F}_{\bpsi}$ by using Stochastic Gradient Acsent (SGA). Algorithm \ref{alg:RandomResidual} summarizes the respective procedure.


\subsection{Form of the Approximating Density $q_{\bpsi}$}
\label{sec:ApproximatingDensity}

%\mc{Until we finalize the form of the covariance matrix I will use this simplified version. As soon as we have obtained good results for the covariance matrix that depends on $\bs{X}$ I will modify the following accordingly.}

In selecting the form of $q_{\bpsi}$ and without loss of generality  we postulate: 
\be
q_{\bpsi}(\bx,\by) = q_{\bpsi}(\by|\bx) q(\bx) = q_{\bpsi}(\by|\bx) p(\bx) %= \mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \boldsymbol{\Sigma}_{\bpsi})~\mathcal{N}\left(\bx | \bs{0}, \bs{I_{d_{\by}}}\right)
\label{eq:AppoxPostForm}
\ee 
i.e. we use the given density of the parametric input and attempt to approximate the input-to-output map with $q_{\bpsi}(\by|\bx)$ where $\bpsi$ denotes the tunable parameters. We note that alternate decompositions might be advisable in the context of inverse problems but are not discussed in this work.
We note also  that a deterministic formulation can be readily adopted by selecting a degenerate density in the form of a Dirac-delta, i.e.:
\be
q_{\bpsi}(\by|\bx)=\delta(\by-\bs{\mu}_{\bpsi} (\bx))
\ee
The sought function $\bs{\mu}_{\bpsi} (\bx)$ in this case can take the form of {\em any }
 of the proposed NN-based architectures such as Fully Connected Neural Networks (FCNNs), Convolutional Neural Networks (CNNs) \cite{zhu2019physics}, Deep Neural Operators (DeepONets) \cite{lu2019deeponet}, Graph Neural Operators (GNOs) \cite{li2020neural} or Fourier Neural Operators (FNOs) \cite{kovachki2021neural}, in which case $\bpsi$ would correspond to the associated NN-parameters.


While all these architectures have produced good results in a variety of problems, it is easily understood that as the variability and the dimension of the input $\bx$ (as well as of the sought output $\by$) increase, so must the complexity of the aforementioned NN-based schemes increase. At a practical level it is not uncommon that one must train for millions or billions of parameters $\bpsi$ (refs). This situation is much more pronounced in {\em multiscale} problems where input and output de facto require high-dimensional representations.


More importantly as such interpolators are agnostic of the physical context, they face significant problems in generalizing (refs). For example if out-of-distribution predictions are sought for a significantly different input $\bx$ as compared to the ones used in training, then the predictive accuracy can significantly drop (refs). In addition and in the context of PDEs in particular, if one were to seek predictions under a different set of boundary conditions than the ones employed during training, most likely, these predictions would be significantly off and by a large margin (see Section \ref{sec:numerical}). 

One could claim that enlarged datasets, or  bigger models or progress in pertinent hardware could alleviate or overcome these difficulties. Nevertheless none of these strategies address the fundamental underlying question which is how to find the requisite information bottlenecks that lead to  drastic dimensionality reductions and lightweight surrogates
 and how to achieve this in a problem-aware manner that is capable of producing accurate  predictions under extrapolative settings \cite{grigo_physics-aware_2019}.



%Given the high-dimensional setting, selecting an appropriate $q_{\bpsi}$ poses significant challenges as this needs to be simultaneously:
%\bi 
%\item \textbf{accurate}, i.e. it should envelop the true $\by$ for each $\bx$ and with the lowest possible uncertainty,
%\item \textbf{generalizable}, i.e. it should be capable of producing accurate predictions for inputs $\bx$ {\em not seen} during training as well as potentially for different boundary conditions or right-hand sides of the governing PDE, and
%\item \textbf{lightweight}, i.e. with a number of parameters $\bpsi$ that, at a minimum, does not grow rapidly with the dimension of the problem.
%\ei 
In view of these objectives and following previous work \cite{grigo_physics-aware_2019,rixner2021probabilistic}, we propose incorporating coarse-grained versions of the governing PDE as an implicit solver \cite{belbute2020combining,um2020solver} in the surrogate constructed. 
We  elaborate on this in the subsequent sections and more importantly we extend this {\em multiscale} problems which pose a unique set of challenges. 
%as previous works has shown, it is advisable  to incorporate as much as possible of the physical structure in $q_{\bpsi}$.
%, we incorporate a coarse-grained version of the reference, fine-grained model. We note that implicit solvers have also been employed in the past as e.g. in \cite{belbute2020combining,um2020solver}.  
For the purposes of the Variational Inference proposed, we employ a multivariate Gaussian of the form:
\be
q_{\bpsi}(\by|\bx)  = \mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \boldsymbol{\Sigma}_{\bpsi})
\label{eq:FormofTheAproxPosterior}
\ee
the mean and covariance of which are discussed in the sequel.
%where $\bs{\mu}_{\bpsi} (\bx)$ is the trainable mean prediction and $\boldsymbol{\Sigma}_{\bpsi}$ is a trainable covariance matrix. From equation \ref{eq:AppoxPostForm}, one can observe that only the mean prediction depends on the inputs. Moreover, the only trainable part of the approximate posterior is the conditional distribution $q_{\bpsi}(\by|\bx)$, which will be ultimately be used for making predictions after training the model. The form of the previous distribution is assumed to be Gaussian, and its parameters are described below. 

\psk{If covariance is described later then there is no reason to have a subsection here}
\subsubsection{Mean function $\bs{\mu}_{\bpsi} (\bx)$}
\label{sec:ApproximatingDensityMu}

In the context of  materials problems and as in the model formulation  of \refeq{eq:DarcyFlowEquation} where the inputs $\bx$ parametrize a, potentially multiscale, material property field,  we consider a (much) coarser, discretized version (see e.g. Figure \ref{fig:CGPhysicsArchitecture}) of the governing PDE where $\bxx, \byy$ denote the respective, discretized input and output. 
By construction, their dimension is much lower as compared to  their reference, fine-grained counterparts $\bx,\by$. As such, the solution of the associated (non)linear algebraic equations to obtain the solution $\byy$ for any input $\bxx$  is much faster.
As we have shown in \cite{grigo_physics-aware_2019}, the $\bxx$ could be thought of as some effective material properties  which serve as the requisite information bottleneck to the  problem. Furthermore, it is possible that  a different (discretized) PDE  could be used as a stencil for the coarse-grained model.
%on the coarse grid. In \cite{grigo_physics-aware_2019} we have shown that even a different PDE could be used as a stencil for the coarse-grained model.

We complement the implicit, differentiable, and vectorized, input-output map  $\byy(\bxx)$  of the CG model, with two additional components:
\bi
\item a fine-to-coarse input map denoted by $\bxx_{\bpsi}(\bx)$ that we express with a shallow CNN parametrized by $\bpsi$ (details in \ref{appendix:shallowCNN}) \psk{Please describe the general structure},
\item a coarse-to-fine output map denoted by $\by(\byy)$ that  attempts to reconstruct the reference, FG output $\by$ given the CG output $\byy$ ( details in \ref{appendix:ytoYTransform}) \psk{Please describe the general architecture}.
\ei
The composition of these three functions, i.e.:
\be
\bs{\mu}_{\bpsi} (\bx)=\by\left( \byy\left(\bxx_{\bpsi}(\bx) \right) \right)
\label{eq:formOfmeanPrediction}
\ee
In the formulation employed in the ensuing numerical experiments, the sole trainable parameters are associated with the inner layer i.e. the fine-to-coarse map from $\bx$ to $\bxx$. More complex formulations involving trainable parameters in the other two layers could be readily accommodated.

We note that all three layers are differentiable, and each evaluation requires a solution of the CG model. Differentiation of $\bs{\mu}_{\bpsi}$ with respect to $\bpsi$ as needed for training requires a backward pass which can be computed with Automatic Differentiation (refs) and/or adjoint formulations of the governing equations of the CG model (Refs).
%for obtaining derivatives.  
The advantages of the adopted model in view of the aforementioned desiderata  will become apparent in the numerical illustrations.


%This term has a particular coarse-grained, physics-retaining form, as shown in figure \ref{fig:CGPhysicsArchitecture}. The coarse-grained (CG) form of $\bs{\mu}_{\bpsi} (\bx)$ is

%\be
%\bx \xrightarrow{f_{\bpsi}(\cdot)} \bs{X} \xrightarrow{G(\cdot)} \bs{Y} \xrightarrow{h(\cdot)} \bs{\mu}_{\bpsi} (\bx)
%\ee
%
%where $f_{\bpsi}(\cdot)$ is a shallow CNN (more details in \ref{appendix:shallowCNN}, responsible for downsampling $\bx$ and learning the most relevant effective properties of $\bx$. After applying $f_{\bpsi}(\cdot)$ a low dimensional representation $\bs{X}$ of the inputs will be used in a fully vectorized and differentiable FEM solver $G(\cdot)$ to find a low dimensional representation of the mean outputs $\bs{Y}$. Lastly, a fixed linear map $h(\cdot)$ is used for acquiring the mean prediction $\bs{\mu}_{\bpsi} (\bx)$ (more details about $h(\cdot)$ in \ref{appendix:ytoYTransform}). The previous architecture allows faster convergence and more precise out-of-distribution predictions, where many state-of-the-art schemes collapse. Furthermore, with very few parameters, it can provide predictions of similar accuracy with state-of-the-art methods while providing uncertainty quantification.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.8\textwidth]{figs/Methodology/physicsSchematicWithMesh.png}
  \caption{Schematic illustration of the proposed, physics-aware procedure for parametrizing the mean solution $\bs{\mu}_{\bpsi} (\bx)$, given an input $\bx$ as described in subsection \ref{sec:ApproximatingDensityMu}. 
  %\psk{It would be good if the meshes good be shown to illustrate the difference in dimension} \mc{Does something like the above suffices?}
  }
  \label{fig:CGPhysicsArchitecture}
\end{figure}

%\psk{Given the different form adopted in 2.8 maybe this can be specialized in the num. illustrations to avoid confusion}
 

\subsection{Tempering of the hyperparameter $\lambda$}
\label{sec:algorithm}

\psk{This paragraph sounds very ad-hoc and suggests that you can select the solution you want at the end without any guiding principle. I suggest you move it after 2.6 and put it as part of a larger section on Algorithmic implementation. 
Therein it should be discussed how SVI is done (i.e. reparametrization trick + MC estimates of the gradient + stochastic gradient ascent) with appropriate references and very technical details moved to an appendix. Tempering could be a part of the overall scheme but it should be motivated appropriately  and a criterion should be defined of when u move to the next lambda.
I.e. algorithm 1 should be included and expanded}.
}
As discussed in \ref{infusingVirtualObservables}, the hyperparameter $\lambda$ controls how strongly the virtual observables will be enforced. This in turn, controls how wide will be the uncertainty bounds of the probabilistic predictions of the trained model. Thus, the selection of $\lambda$ is ultimately selected by the user of the algorithm, according to the respective objectives. Ultimately, the optimal $\lambda$ is different for each case it is up to the user to run a short calibration process to determine what $\lambda$ will result in the best suited for the problem uncertainty bounds range.


\begin{algorithm}[H]
% \caption{Simple Description of the Learning Algorithm.}
\begin{algorithmic}[1]
    \State  $\bpsi\gets \boldsymbol{\psi_0}$; \Comment{Initialization of $\boldsymbol{\psi}$}
\While{$\mathcal{F}_{\bpsi}$ not converged} 
   \State $k \sim Categorical\left(p=\frac{1}{N}\right)$; \Comment{Drawing random $k$}
   \State  $\bx_{m}, ~ \by_{m} \sim q_{\boldsymbol{\psi}}(\bx, \by), ~~~~ m = 1, 2, ..., M$ 
   \State Estimate $\nabla_{\bpsi} \mathcal{F}_{\bpsi}$ \Comment{
    %\gets \frac{1}{M}\sum_{n_m=1}^{N_m}\hat{\mathcal{F}}(q_{\bpsi}(\bx_{n_m},\by_{n_m}), \hat{\boldsymbol{\phi}}_{max})$ // 
    \textbf{Monte Carlo} estimate of $\nabla_{\bpsi} \mathcal{F}_{\bpsi}$  with \textbf{Reparameterization trick}} %estimate of $\hat{\mathcal{F}}$
    \State $\bpsi_{\ell+1} \gets \bpsi_{\ell} + \boldsymbol{\rho}^{(\ell)} \odot \nabla_{\bpsi} \mathcal{F}_{\bpsi}$ \Comment{ \textbf{SGA  using ADAM} }
    \State $\ell \gets \ell + 1$
\EndWhile
\end{algorithmic}
\caption{Random Residual Algorithm.}
%\caption{Assuming $q_{\bpsi}(\bx,\by)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T)~\mathcal{N}\left(\bx | \bs{0}, \bs{I}\right)$ }
\label{alg:RandomResidual}
%\psk{Algorithms should come after the full model has been presented}
\end{algorithm}


\subsection{Predictions}

After training has finished, the density $q_{\bpsi}(\by|\bx)$ that has been obtained can be used for providing predictions. Samples can be drawn from $q_{\bpsi}(\by|\bx)$ because of its Gaussian form. For any given input $\bx$, the mean coefficients of the solution are given from Equation \eqref{eq:formOfmeanPrediction}. The previous samples and the mean coefficients can be easily converted to the respective fields by using the representation shown in Equation \eqref{eq:trialSolRepresentation} (see subsection \ref{sub:2D_Darcy}). The variance of the predicted field can be determined empirically from the previous samples, and in turn, one can obtain the upper and lower uncertainty bound of the solution for any given $\bx$. The process for obtaining probabilistic predictions is shown in Algorithm \ref{alg:MakingPredictions}.

\begin{algorithm}[H]
% \caption{Simple Description of the Learning Algorithm.}

%Given a single input $\bx$ for which we wish to make a prediction:\;

\begin{algorithmic}[1]
    \State {$u_{\mu}(\bs{s}) \leftarrow \sum_{i=1}^{N_{\eta}} \mu_{\bpsi} (\bx)_i \eta_i(\bs{s})$} \Comment{Mean Solution Field}
    \For{$j=1$ to $J$}
    \State {Sample $\by^{(j)} \sim q_{\bpsi}(\by|\bx)$\;}      \Comment{$q_{\bpsi}(\by|\bx)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \boldsymbol{\Sigma}_{\bpsi})$}
    \State {$u^{(j)}(\bs{s}) = \sum_{i=1}^{N_{\eta}} y_i^{(j)} \eta_i(\bs{s})$} \Comment{Reconstruction of the Solution fields (see Equation \ref{eq:trialSolRepresentation})}
    \EndFor
    \State $u_{\sigma}(\bs{s}) \leftarrow \sqrt{ \sum_{j=1}^J \frac{\left( u^{(j)}(\bs{s}) - u_{\mu}(\bs{s})\right)^2}{J-1}}$ \Comment{Standard Deviation of the Solution Field}
    \State $u_{U}(\bs{s}) \leftarrow u_{\mu}(\bs{s}) + 2 u_{\sigma}(\bs{s})$ \Comment{Upper Uncertainty Bound Field}
    \State $u_{L}(\bs{s}) \leftarrow u_{\mu}(\bs{s}) - 2 u_{\sigma}(\bs{s})$ \Comment{Lower Uncertainty Bound Field}
    
\end{algorithmic}
\caption{Making Predictions for a single input $\bx$}
%\caption{Assuming $q_{\bpsi}(\bx,\by)=\mathcal{N}(\by|\bs{\mu}_{\bpsi} (\bx), \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T)~\mathcal{N}\left(\bx | \bs{0}, \bs{I}\right)$ }
\label{alg:MakingPredictions}
%\psk{Algorithms should come after the full model has been presented}
\end{algorithm}

To assess the performance of the proposed model and compare it objectively with other state-of-the-art models, we consider a validation dataset $\mathcal{D}_v = \{ \mathbf{x}^j, \mathbf{y}^j \}_{j=1}^{N_j}$ consisting of $N_j$ input-output pairs, which were obtained by using a conventional FEM solver on a fine mesh. Subsequently, the following metrics will be employed:

\textbf{Coefficient of Determination $R^2$:}
The coefficient of determination is a widely used metric \cite{coeffDetermZhang} to quantify the accuracy of point estimates and it is defined as follows

\begin{equation}
R^2 = 1 - \frac{\sum_{j=1}^{N_j} \| \by_j - \mu(\bx_j) \|_2^2}{\sum_{j=1}^{N_j} \| \by_j - \bar{\by} \|_2^2}
\end{equation}

where $\mu(\bx_j) = \mathbb{E}_{q_{\bpsi}(\by | \bx)} \left[ \by \right]$ is the mean of the predictive posterior $q_{\bpsi}(\by|\bx)$ of our trained model for each point $\bx_j$ and $\bar{\by} = \frac{1}{N_j} \sum_{j=1}^{N_j} \by_j$ is the sample mean of the validation dataset. According to the previous metric, the best possible prediction accuracy is attained when $R^2=1$. It is noted that negative $R^2$ values are also valid since the second term is merely weighted (not bounded) by the empirical variance of the validation dataset.

\textbf{Relative $L_2$ Error $\epsilon$:} The relative $L_2$ error is commonly used as an evaluation metric for comparisons between state-of-the-art surrogate models for stochastic PDEs \cite{zhu2019physics, lu2022comprehensive, wang2021learning}. The definition is given by

\begin{equation}
\epsilon = \frac{1}{N_j} \sum_{j=1}^{N_j}\frac{ \| \by_j - \mu(\bx_j) \|_2}{\| \by_j \|_2}.
\end{equation}
%\textbf{Enveloping Score $M_e$:}


%\psk{Don't u show predictive estimates based on $q(\by|\bx)$ as well? An algorithm should be added that explains how these predictive estimates are generated see e.g. \cite{rixner2021probabilistic} Alg. 2.}


==> section3/1_GeneralSetupDescription.tex <==



\section{Numerical Illustrations}
\label{sec:numerical}

In this section, the proposed framework's capabilities and advantages are demonstrated in a series of different setups. Additionally, the components of the model described in the previous sections are further specified with the main implementation details. More specifically, the numerical illustrations aim:

\begin{itemize}
    \item to assess the predictive performance of the proposed framework and compare it with a state-of-the-art physics-informed method (Physics Informed Fourier Neural Operators (PINO) \cite{li2021physics}). The above comparison is conducted in the context of a parametric linear Poisson PDE (2D Darcy Flow Problem).
    \item to demonstrate the excellent extrapolative behavior of the proposed model in various out-of-distribution conditions, in which other surrogate models like PINO fail to resolve the solution accurately. These involve significantly different boundary conditions and volume fractions (for the 2 phase medium) than the ones used for training.
    \item to examine the performance of the model on non-linear parametric PDEs.
    \item to showcase the ability of the method described in subsection \ref{sec:CGLearning} to efficiently discover the low dimensional solution manifold, when the input is high dimensional, by using as the only source of information the residual. To our knowledge, this is the first time that this is achieved.
    \item to illustrate the superior performance of the above lightweight model for high dimensional input fields that involve very fine fluctuations, and compare it with state-of-the-art deep learning operator methods, which involve millions of trainable parameters.
\end{itemize}

% \psk{Potential additions: \\
% \bi
% \item Illustrations of pairs of $\bx$ and $\bxx$ after training could provide insight. 
% \item Potentially an illustration with respect to the number of inputs $\bx$ used during training would be useful. The goal would be to show how quickly the model saturates and is able to provide accurate predictions. This could be combined with the multiscale setting.
% \ei
% }

\subsection{High Dimensional Darcy Problem} \label{sub:2D_Darcy}
To demonstrate the predictive capabilities of our framework we select the following Darcy flow equation with zero Dirichlet conditions on every boundary

\begin{equation}
\begin{array}{lll}
 \nabla \cdot \left( - c(\bs{s}, \bx) \nabla  u(\bs{s})\right) = f, ~~~ \mathbf{s} \in \Omega = \left[0, ~ 1 \right] \times\left[0, ~ 1 \right] \\
u(\bs{s}) = u_0, ~~~ \mathbf{s} \in \Gamma_D
\end{array}
\label{eq:2D_Darcy}
\end{equation}

\noindent This setup has been used for illustration purposes in many state-of-the-art methods \cite{li2020fourier} \cite{li2021physics} \cite{lu2022comprehensive} and the respective code was already available for producing the following comparative figures. The target is to create an accurate forward map between the conductivity field $c(\bs{s}, \bx)$ and the solution $u(\bs{s})$ of the PDE or equivalently an accurate map from the input parameters $\bx$ to the output parameters $\by$. For all the following illustrations, the external force term will be set to $f=100$ for all the following illustrations.

To produce the conductivity fields, i.e. the input dataset used for training from the inputs we use a Gaussian Random Field (GRF). Firstly, an intermediate conductivity field  $G(\mathbf{s}) \sim \mathcal{GP}\left(0, ~ k(\mathbf{s}, \mathbf{s}^{\prime}) \right)$ is produced, where $k(\mathbf{s}, \mathbf{s}^{\prime}) = exp\left(-\frac{||\mathbf{s}-\mathbf{s}^{\prime}||^2_2}{l^2}\right)$ and $l$ is the length scale. In order to parameterize the previous field by using $\bx \sim \mathcal{N}\left(\mathbf{0}, \mathbf{I}\right)$, we use the Karhunen-Lo\`{e}ve Expansion (KLE) and thus $G(\bs{s}, \bx) = \sum_{i=1}^{dim(\bx)} \sqrt{\lambda_i} x_i \mathbf{V}_i$, where $\lambda_i$ are the eigenvalues and $\mathbf{V}_i$ the eigenvectors of $k(\mathbf{s}, \mathbf{s}^{\prime})$. More details about the previous process can be found in \cite{zhu2018bayesian} and \cite{zhu2019physics}, where a slightly different kernel was used. Furthermore, we convert $G(\mathbf{s})$ to a two-phase medium by applying the following equation

\be
c(s_i, \bx) = \begin{cases} 1, ~G(s_i, \bx) \ge t \\ \frac{1}{CR}, ~G(s_i, \bx)< t \end{cases} 
\ee

The threshold $t$ is chosen according to the volume fraction of phases that we would like to achieve in the medium For example, for achieving a volume fraction (VF) of $50 \%$ we should set $t=0$. $CR$ is the contrast ratio between the phases and in general, the higher $CR$ is the more difficult it is to obtain accurately the PDE solution.

\textbf{Fine-Grained Model (FGM):}
The FGM is used only for producing the reference solution to assess the performance of the proposed or other models. The Fenics open-source software \cite{fenics2015} was used for this purpose. The used uniform mesh consists of $Nf=8192$ regular, linear, and triangular elements. The conductivity field is given as the input to the solver in the form of nodal values. However, the solver uses only the conductivity value at the centroid of each triangle to solve the PDE.

\textbf{Coarse Grained Model (CGM):}
The CGM is used exclusively in our framework as an informational bottleneck. The structure of the mesh and all the details remain the same as in the FGM, except from the number of elements $Nc$ used in each experiment, which will be stated explicitly for every experiment. Furthermore, the implementation of the solver was coded from scratch and doesn't rely at all on Fenics, even though it gives identical results. This was done to ensure that the CGM is fully vectorizable and differentiable. The previous two properties were necessary for leveraging the full computational power of modern GPUs and for having easy access to the gradients by using Auto-differentiation.

\textbf{Weighted Residual Specification:}
In section \ref{sec:SWform}, we generally derived the weak form of the residual that will be used as virtual observables for training the framework. The weighting functions of the weak form need to be specified in two separate levels in the context of this framework. The first level involves the CGM mentioned above, where the used shape functions are the traditional triangular finite element shape functions, denoted by the vector $\bs{\Phi}(\bs{s}) = \{\Phi_m(\bs{s}) \}_{m=1}^{N_c}$, where each function $\Phi_m (\bs{s})= \sum_{i=1}^3 \phi_{i, loc}^{m} \Phi_{i, loc}^{m}(\bs{s})$ is computed by using the three respective shape functions for each triangular element. This approach leads to the following $N_c$ in total weighting functions:

\begin{equation}
w(\bs{s}) = \sum_{m=1}^{N_c} \phi_m \Phi_m(\bs{s}), ~~~ m=1,2,3,...,N_c
\end{equation}

\noindent where $\phi_{i, loc}^m$ and $\Phi_{i, loc}^{m}(\bs{s})$ are the $i_{th}$ coefficient and shape function respectively of the local $m_{th}$ element and $\phi_m$ is the equivalent global $m_{th}$ coefficient.

The second level involves the calculation of the FGM residual. These residuals drive the maximization of the ELBO by entering randomly in the likelihood term of \refeq{eq:elboRandomResidual}. The weighting functions, in this case, are represented as follows:

\begin{equation}
    w(\bs{s}) = \sum_{i=1}^{N_{\xi}} \phi_i \xi_i(\bs{s}), ~~~ i=1,2,3,...,N_f
\end{equation}

\noindent where $\phi_i$ are the respective coefficients and $\xi(\bs{s})$ are Radial Basis Functions (RBFs) given by the following formula:

\begin{equation}
    \xi_i(\bs{s}) = \tau(\bs{s})exp\left( \frac{|| \bs{s} - \bs{s_{i,0}}||^2_2}{\Delta l_{\xi}^2} \right)
\end{equation}

\noindent where $\bs{s_{i,0}}$ is the center of each individual RBF and $\Delta l_{\xi}$ is a scale parameter. After empirical observations we concluded that $\Delta l_{\xi} = \frac{1}{\sqrt{N_{\xi}}-1}$ is a sufficient choice. The above configuration of weight functions in a unit-squared domain involves a uniformly distributed grid of nodes $\bs{s_{i,0}}$, where each one defines its respective RBF. The term $\tau(\bs{s})=\bs{s}_x\bs{s}_y(\bs{s}_x-1)(\bs{s}_y-1)$ is required to ensure that every weight function will have zero values at the boundary, as required from the previous definition of the problem. Some indicative random sets of the above weighting functions, in accordance with the algorithm \ref{alg:RandomResidual}, are presented in Figure \ref{fig:randomlySelectedRbfs}.

The representation of the trial solution is given by
\begin{equation}
    u(\bs{s}) = \sum_{i=1}^{N_{\eta}} y_i \eta_i(\bs{s}), ~~~ i=1,2,3,...,N_{\eta}
    \label{eq:trialSolRepresentation}
\end{equation}

\noindent where $y_i$ are the respective coefficients and $\eta(\bs{s})$ are RBFs defined as
\begin{equation}
    \eta(\bs{s})=exp\left( \frac{|| \bs{s} - \bs{s_{i,0}}||^2_2}{\Delta l_{\eta}^2} \right)
\end{equation}

\noindent where $\Delta l_{\eta} = \frac{1}{\sqrt{N_{\eta}}-1}$.

It is clear from the above that the number of the RBFs used for the weighting functions ($N_{\xi}$) and the trial solution ($N_{\eta}$) can also be different. This is in fact true in the following illustrations of the current subsection, where it isn't true for subsection $\ref{sub:CGLearningIllustrations}$.


\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/randShapeFunctions/randShapeFuncs10.png}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/randShapeFunctions/randShapeFuncs100.png}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/randShapeFunctions/randShapeFuncs500.png}
    \end{minipage}
    \caption{Illustration of 10, 100, and 500 randomly selected RBF-based weighting functions according to algorithm \ref{alg:RandomResidual}. Each one of these RBFs corresponds to a single residual where the governing equations are enforced.}
    \label{fig:randomlySelectedRbfs}
\end{figure}

\textbf{Posterior covariance matrix $\boldsymbol{\Sigma}_{\bpsi}$:} The covariance matrix $\boldsymbol{\Sigma}_{\bpsi}$ presented in Equation \ref{eq:FormofTheAproxPosterior} is specified for the following illustrations as:

\begin{equation}
\boldsymbol{\Sigma}_{\bpsi} = \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T+\sigma_{\bpsi} \mathbf{I}_{d_{\by}}
\end{equation}
while $\bs{L}_{\bpsi}$ is a reduced order matrix of dimensions $\left(d_{\by},~ K\right)$ and $\sigma_{\bpsi}^2$ is a global Gaussian noise. The first term is responsible for introducing some correlation between the different spatial points of the solution. Meanwhile, a full covariance matrix is avoided to keep the dimension of the parameters low. The second term is introduced to efficiently capture the global uncertainty in the solution prediction. Thus, the reparameterization trick, when sampling for $\by$ has the following form

\be
\by \sim \bs{\mu}_{\bpsi} (\bx) + \bs{L}_{\bpsi} \bs{\varepsilon_1} + \sigma_{\bpsi} \bs{\varepsilon_2}, ~~~ \bs{\varepsilon_1} \sim \mathcal{N}\left( \bs{0}, ~ \bs{I_K} \right),  ~ \bs{\varepsilon_2} \sim \mathcal{N}\left( \bs{0}, ~ \bs{I_{d_{\by}}} \right)
\ee

where $dim(\bs{\varepsilon_1})=K$, $dim(\bs{\varepsilon_2})=d_{\by}$.

==> section3/2_differentVolumeFractions.tex <==
\subsection{Comparison for Different Volume Fractions}

In the following illustrations will use the following two datasets $A=(CR=10,~ VF=50 \%, u_0=0)$ and $B=(CR=10,~ VF=90 \%, u_0=0)$. In order to demonstrate the superior performance of the model in extrapolative conditions, both the coarse-grained surrogate and PINO are trained on dataset A and tested on dataset B. The performance of the two models is similar for in-distribution predictions. The mean prediction in both cases is close to the ground truth as seen from the coefficient of determination $R^2$. However, the proposed framework provides uncertainty bounds for the predicted solution, in contrast to PINO, which provides only point estimates for the PDE solution.

When the same models are inquired in out-of-distribution conditions (different volume fraction), the suggested coarse-grained surrogate retains fully the prediction accuracy, while the predictive accuracy of PINO collapses in the same scenario. As seen from figure \ref{fig:DiffVFs}, the coarse-grained surrogate retains its predictive accuracy for every possible volume fraction, as opposed to PINO, of which the accuracy decreases significantly as the volume fraction deviates notably from the one used for training. The previous behavior can be attributed to the physics-inspired structure that the mean prediction $\boldsymbol{\mu}_{\bpsi}(\bx)$ has.


\begin{figure}[H]
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/Darcy_pwc/elbo.png}
        \caption{Convergence of the Loss function (ELBO) for the coarse-grained surrogate, when trained on $VF=50\%$.}
        \label{fig:ELBOconvergence}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/Darcy_pwc/diffVF.png}
        \caption{Predictive Accuracy of the coarse-grained surrogate and PINO for various volume fractions when trained on $A=(CR=10,~ VF=50 \%, u_0=0)$.}
        \label{fig:DiffVFs}
    \end{minipage}
\end{figure}

\begin{figure}[H]
    \centering
    \subfigure[Coarse-grained surrogate trained and tested on dataset A.]{
        \includegraphics[width=0.9\linewidth]{figs/Darcy_pwc/VF_50_to_50.png} % Replace 'placeholder_image' with your image file
    }
    
    \vspace{1cm} % Add vertical space between rows
    \subfigure[\textbf{Out of distribution Prediction:} Coarse-grained surrogate trained dataset A and tested on dataset B.]{
        \includegraphics[width=0.9\linewidth]{figs/Darcy_pwc/VF_50_to_90.png}
    }
    
    \caption{Comparison between the Random Residual Algorithm described in subsection \ref{sec:GreedyAlgorithm} and the Physics Informed FNO (PINO) \cite{li2021physics}.}
\end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/Darcy_pwc/diffVF.png} % Replace 'placeholder_image' with your image file
%     \caption{Predictive Accuracy of the coarse-grained surrogate and PINO for various volume fractions when trained on $VF=50\%$.}
%     \label{fig:DiffVFs}
% \end{figure}


==> section3/3_differentBoundaryConditions.tex <==
\subsection{Comparison for Different Boundary Conditions}

In the following illustrations, we will focus on another difficult extrapolative setup, which requires the compared model to predict in cases where the boundary conditions are drastically different from the ones used to train the models. In figure 

In the following illustrations will use the following two datasets $A=(CR=10,~ VF=74 \%, u_0=0)$ and $C=(CR=10,~ VF=74 \%, u_0=10)$. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/Darcy_pwc/D0toDsinx.png}
    \caption{Comparison between the Random Residual Algorithm descibed in subsection \ref{sec:GreedyAlgorithm} and the Physics Informed FNO (PINO) \cite{li2021physics}.}
\end{figure}

\begin{table}[H]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    Boundary Condition Type & MAE (PINO) & MAE (CG model) \\
    \hline
    $u=0$ everywhere & $??$ & $??$ \\
    \hline
    $u=10$ everywhere & $??$ & $??$ \\
    \hline
    $u=sin(2 \pi t), ~ t\in [0, 1]$ along the boundary  & $??$ & $??$ \\
    \hline
  \end{tabular}
  \caption{Comparison of Mean Absolute Error (MAE) between each model and the ground-truth for Different Boundary Conditions. }
  \label{tab:CGLearningVSPINOdiffBCs}
\end{table}

==> section3/4_CGLearning.tex <==
\subsection{Coarse-Grained Learning}
\label{sub:CGLearningIllustrations}

In this subsection, we show the impact of applying the formulations described in subsection \ref{sec:CGLearning}. For this purpose, we decreased the correlation length of the used GRFs to $l=0.05$ from $l=0.25$, which was the case for the previous illustrations. This change results in a conductivity field of multiple scales, such as the ones shown in figure \ref{}. It is clear that for such conductivity fields, the solution will mostly have a simple low-frequency form upon which other high-frequency components will be present.

The Posterior covariance matrix $\boldsymbol{\Sigma}_{\bpsi}$ in this setup is given by:

\begin{equation}
\boldsymbol{\Sigma}_{\bpsi} = \bs{L}_{\bpsi}\bs{L}_{\bpsi}^T+\sigma_{\bpsi} \mathbf{I}_{d_{\bs{Y}}}
\end{equation}
while $\bs{L}_{\bpsi}$ is a reduced order matrix of dimensions $\left(d_{\bs{Y}},~ K\right)$ and $\sigma_{\bpsi}^2$ is a global Gaussian noise. The form is essentially the same as the one discribed in subsection \ref{sub:2D_Darcy}, with the only difference that the perturbations are now applied on $\bs{Y}$ instead of $\bs{y}$. Thus, the reparameterization trick, when sampling for $\bs{Y}$ will have the following form

\be
\bs{Y} \sim \bs{\mu}_{\bpsi} (\bx) + \bs{L}_{\bpsi} \bs{\varepsilon_1} + \sigma_{\bpsi} \bs{\varepsilon_2}, ~~~ \bs{\varepsilon_1} \sim \mathcal{N}\left( \bs{0}, ~ \bs{I_K} \right),  ~ \bs{\varepsilon_2} \sim \mathcal{N}\left( \bs{0}, ~ \bs{I_{d_{\bs{Y}}}} \right)
\ee

where $dim(\bs{\varepsilon_1})=K$, $dim(\bs{\varepsilon_2})=d_{\bs{Y}}$.

In figure \ref{fig:CGLearningWandWO}, the proposed framework with and without the modification described in subsection \ref{sec:CGLearning} was employed to learn the dependence of the coarse-grained solution $\by_c$ on $\bx$. The first is quite successful in learning the map, unlike the second one, which fails. Also, the predicted solution has a relatively low absolute error, compared to the true solution, even though, the difference between the degrees of freedom of the coarse and fine representation is approximately two orders of magnitude.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/CGLearning/CGLearningWandWO.png}
    \caption{The prediction of the proposed framework, with and without applying the method described in \ref{sec:CGLearning}.}
    \label{fig:CGLearningWandWO}
\end{figure}

The assumptions made in subsection \ref{sec:CGLearning} regarding the quick saturation of proposed model are further supported from the experiments presented in figure \ref{fig:CGLearningSaturation}. One can see that the relative error, is quite low even if only one input instance of $\bx$ is used ($K=1$). The prediction performance improves in an asymptotic fashion, so that we could state that after $K=100$ a significant improvement in performance isn't observed anymore. \mc{Furthermore ...}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/CGLearning/CGLearningVSPINO.png}
    \caption{Comparision between the proposed framework and PINO for conductivity fields with $l=0.05$ (\textbf{In-distribution predictions}.}
    \label{fig:CGLearningSaturation}
\end{figure}

Finally, we will illustrate the superior performance of the proposed surrogate model in these kinds of setups by comparing with a state-of-the-art surrogate model which tries to resolve the map between the input and the full-order output. For this purpose, we employ PINO again \mc{(Potentially I could even use just FNO to make my point stronger)} which involves $2.5$ million parameters. The results of the comparison are depicted in figure \ref{fig:CGLearningVSPINO} and the most important parameter of the two models in table \ref{tab:CGLearningVSPINO}. \mc{Despite the one order difference in training time (wall clock time in the same machine) the two models have similar accuracy...}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/CGLearning/CGsaturationX.png}
    \caption{CG model saturation with the number of inputs $\bx$ used during training.}
    \label{fig:CGLearningVSPINO}
\end{figure}


\begin{table}[H]
  \centering
  \begin{tabular}{|c|c|}
    \hline
    Variable & Dimension (Reference) \\
    \hline
    $\mathbf{x}$ & $1024$ \\
    \hline
    $\mathbf{y}$ & $4096$ \\
    \hline
    $\mathbf{X}$ &  $81$ \\
    \hline
    $\mathbf{Y}$ & $81$ \\
    \hline
  \end{tabular}
  \caption{Most important dimensions of the two models.}
  \label{tab:CGLearningVSPINO}
\end{table}

Moreover, in tables \ref{tab:CGLearningDiffVF} and \ref{tab:CGLearningVSPINOdiffBCs}, the superior extrapolation capabilities of the proposed framework are demonstrated. Even though the previous model was trained for a single pair of volume fraction and boundary conditions $(VF=50 \%, ~ u_{BC}=0)$ it is able to maintain its predictive accuracy in very different setups of boundary conditions and volume fractions, unlike PINO which gives very poor predictions in the above setups.

\begin{table}[H]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    Volume Fraction (VF) & MAE (PINO) & MAE (CG model) \\
    \hline
    $10 \%$ & $??$ & $??$ \\
    \hline
    $30 \%$ & $??$ & $??$ \\
    \hline
    $50 \%$ & $1.475$ & $1.155$ \\
    \hline
    $70 \%$ & $??$ & $??$ \\
    \hline
    $90 \%$ & $??$ & $??$ \\
    \hline

  \end{tabular}
  \caption{Comparison of Mean Absolute Error (MAE) between each model and the ground-truth for Different Volume Fractions}
  \label{tab:CGLearningDiffVF}
\end{table}


\begin{table}[H]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    Boundary Condition Type & MAE (PINO) & MAE (CG model) \\
    \hline
    $u=0$ everywhere & $1.475$ & $1.155$ \\
    \hline
    $u=10$ everywhere & $??$ & $??$ \\
    \hline
    $u=sin(2 \pi t), ~ t\in [0, 1]$ along the boundary  & $??$ & $??$ \\
    \hline
  \end{tabular}
  \caption{Comparison of Mean Absolute Error (MAE) between each model and the ground-truth for Different Boundary Conditions. }
  \label{tab:CGLearningVSPINOdiffBCs}
\end{table}

Finally, one could draw some intuition conclusions from figure \ref{fig:CGLearningxXpairs}. For each full input $x$, the model learns a coarse-grained input $X$, which gives the best possible score in terms of the residual. For inputs that contain very fine fluctuations, the model distinguishes a properly weighted coarse approximation. In other words, during this stage, the input is downsampled properly but at the same time, the proper conductivity scale of the input is learned that best fits the solution according to the residual.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/CGLearning/CGLearningxXpairs.png}
    \caption{Multiple pairs of the full input $x$ and the learned coarse-grained input $X$.}
    \label{fig:CGLearningxXpairs}
\end{figure}

==> section3/5_NonLinearPoisson.tex <==
\subsection{Non-Linear Poisson Equation}

In this subsection, we assess the performance of the proposed model on non-linear PDEs. It will be apparent that the model's behavior presented in the previous chapter is not limited to linear PDEs, but it also applies in a non-linear PDE setup. For this purpose, the model is trained to predict the solution of the following parametric non-linear PDE.

\begin{equation}
\begin{array}{lll}
\nabla \cdot  \bs{q}  = f, ~~~ \mathbf{s} \in \Omega = \left[0, ~ 1 \right] \times\left[0, ~ 1 \right] \\
u(\bs{s}) = u_0, ~~~ \mathbf{s} \in \Gamma_D
\end{array}
\label{eq:nonLinearPDE}
\end{equation}

\noindent and the non-linear constitutive law is

\begin{equation}
\bs{q} = - c(\bx, \bs{s}) e^{\alpha (u(\bs{s}) - u_0)}~ \nabla u
\end{equation}

\noindent where $c(\bx, \bs{s})$ is as in subsection \ref{sub:2D_Darcy}, and $\alpha$, $u_0$ are two additional parameters (assumed to be independent of $\bs{s}$. It is noted that $\alpha$ (and secondarily $u_0$) controls the degree of non-linearity. For $\alpha = 0$, equation \ref{eq:nonLinearPDE}, will take the same form as in equation \ref{eq:2D_Darcy}.

The surrogate model is trained for $l=0.25$ and $l=0.05$ by using the residual from the aforementioned non-linear stochastic PDE. The formulations described in subsection \ref{sec:CGLearning} are employed only when $l=0.05$. The predictive performance is shown in figure \ref{fig:NonLinearl025andl005}. The accuracy of the prediction remains high in both cases, demonstrating that the proposed framework, can be used effectively in non-linear stochastic PDEs too.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figs/CGLearning/CGLearningWandWO.png}
%     \caption{Prediction for the non-linear PDE of equation \ref{eq:nonLinearPDE}. The length scale of the conductivity field is $l=0.25$ (left) and $l=0.05$ (right).}
%     \label{fig:NonLinearl025andl005}
% \end{figure}

\begin{figure}[H]
    \centering
    \begin{minipage}[b]{0.85\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/nonLinearPDE/l025.png}
    \end{minipage}
    \vspace{1.cm}
    \begin{minipage}[b]{0.85\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/nonLinearPDE/l025.png}
    \end{minipage}
    \label{fig:NonLinearl005}
    \caption{Prediction for the non-linear PDE of equation \ref{eq:nonLinearPDE} with $l=0.25$ (top) and $l=0.05$ (bottom).}
\end{figure}
